Compositional Transformers for Scene Generation

We introduce the GANformer2 model, an iterative object-oriented transformer, explored for the task of generative modeling. The network incorporates strong and explicit structural priors, to reflect the compositional nature of visual scenes, and synthesizes images through a sequential process. It operates in two stages: a fast and lightweight planning phase, where we draft a high-level scene layout, followed by an attention-based execution phase, where the layout is being refined, evolving into a rich and detailed picture. Our model moves away from conventional black-box GAN architectures that feature a flat and monolithic latent space towards a transparent design that encourages efficiency, controllability and interpretability. We demonstrate GANformer2's strengths and qualities through a careful evaluation over a range of datasets, from multi-object CLEVR scenes to the challenging COCO images, showing it successfully achieves state-of-the-art performance in terms of visual quality, diversity and consistency. Further experiments demonstrate the model's disentanglement and provide a deeper insight into its generative process, as it proceeds step-by-step from a rough initial sketch, to a detailed layout that accounts for objects' depths and dependencies, and up to the final high-resolution depiction of vibrant and intricate real-world scenes. See https://github.com/dorarad/gansformer for model implementation.

==> draft.tex <==
% ***** into start


% somwhat, quite, 
% ren
%  interpretability 
%  [and the understanding and interpretability of the underlying synthesis process the generative model remains limited].  
% the particularities of the transformation/mapping 

% [largely]
% / properties
% [degree of]
% stunning/impressive photorealistic mainly of single-objects,.. impressi
% more complicated and complex 
% modifying the a particular



% simply mapping a vector of random noise into image space
% an entire scene in an unfactored fashion
% and almost-indistinguishable
% intrinsic structure
% mechanisms
% thereby 
% fail to 
% (3)(1)(1)(2)(3)  
% from a random latent vector to the 
% /natural


% some indication/evidence for disentanglement of global factors/axes of variation / properties 
% Deep generative models [Goodfellow et al., 2014] have been used to synthesize realistic images and learn rich internal representations. Representations learned by these methods are typically hard for humans to interpret and understand

% Recently, generative adversarial networks (GAN) [6] have shown stunning results in generating photorealistic images of faces [16, 17] and simple objects [34, 1, 22]. However, generating photorealistic images for complex scenes with different types of objects and stuff remains a challenging problem. 

% The resolution and quality of images produced by generative methods — especially generative adversarial networks (GAN) [22] — have seen rapid improvement recently [30, 45, 5]. Yet the generators continue to operate as black boxes, and despite recent efforts [3], the understanding of various aspects of the image synthesis process, e.g., the origin of stochastic features, is still lacking. The properties of the latent space are also poorly understood, and the commonly demonstrated latent space interpolations [13, 52, 37] provide no quantitative way to compare different generators against each other.

% Even so, there lacks enough understanding of how GAN connects the latent space and the image semantic space, as well as how the latent code can be used for image editing.

% Yet, Traditional

% Deep generative models allow for photorealistic image synthesis at high resolutions. But for many applications, this is not enough: content creation also needs to be controllable

% Further, only few works consider the compositional nature of scenes. 

% However, realistic images have complicated intrinsic structures and most DGMs fail to consider these structures by simply mapping a vector of random noise into image space.

% While 2D generative adversarial networks have enabled high-resolution image synthesis, they largely lack an understanding of the 3D world and the image formation process

% explicit spatial interaction between multiple entities that could be present in a scene. Capturing such complex interactions between different objects in the world, including their relative scaling, spatial layout, occlusion, or viewpoint transformation is a challenging problem

% lack sufficient mechanisms semantic integrity for the training of deep models.

% Despite the recent advance of Generative Adversarial Networks (GANs) in high-fidelity image synthesis, there lacks enough understanding of how GANs are able to map a latent code sampled from a random distribution to a photorealistic image.

% However, it is uncertain how semantics originate and are organized in the latent space. 

% However, in most practical applications, GAN models are typically used as black-box instruments without a complete understanding of the underlying generation process

% Recent advance of Generative Adversarial Networks (GANs) [11, 16, 17, 6] is capable of transforming random noises into high-quality images, however, the nature of the learned generative representations and how a photorealistic image is being composed over different layers of the generator in GAN remain much less explored

% The vast majority of such models use a monolithic, unstructured latent space, that represents an entire scene in an unfactored fashion

% contemporary

% However, most deep learning models do not explicitly or directly reflect this compositionality so common in the world around us. Most approaches to automatic image generation, however, aim to generate entire scenes at once. Standard GAN: Latent -> image. 
% Issues (1) Lack of structure and interpretability, one latent, conseqneutaly: (2) output image usually are single object (2) lack of control, editability and disentanglement 

% The monolithic structure of the latent space doesn’t offer easy means for controllability disentanglement of interpretability at the object level of specific regions

% deep learning models in contrast. 

% Yet, most deep learning approaches learn distributed representations that do not capture the compositional properties of natural scenes. 

% Deep generative models have shown promising results in generating realistic images, but it is still non-trivial to generate images with complicated structures. The main reason is that most of the current generative models fail to explore the structures in the images including spatial layout and semantic relations between objects. 

% “flat” vector representations that fail to capture the compositional structure of natural scenes

% At lower resolutions or in specialized domains, GAN-based methods are able to synthesize samples which are near-indistinguishable from real samples [7]. However, generating complex, high-resolution scenes from scratch remains a challenging problem. As image resolution and complexity increase, the coherence of synthesized images decreases — samples contain convincing local textures, but lack a consistent global structure.

% However, despite recent breakthroughs in computer vision fuelled by advances in deep learning, learning to represent realistic visual scenes in terms of objects remains an open challenge for artificial systems. 

% These methods give stunning results but struggle to faithfully reproduce complex sentences with many objects and relationships.
% internal representations


% However, these approaches ignore one of the most basic underlying principles of image formation. Images are a product of two separate phenomena: Structure: this encodes the underlying geometry of the scene. It refers to the underlying mesh, voxel representation etc. Style: this encodes the texture on the objects and the illumination.

% In the context of generative neural networks, this typically means that all the pixels are conditioned on a single latent distribution 

% ●	Despite this tremendous success, many questions remain to be answered. For example, to produce a church image (Figure 1a), what knowledge does a GAN need to learn? Alternatively, when a GAN sometimes produces terribly unrealistic images (Figure 1f), what causes the mistakes? Why does one GAN variant work better than another? What fundamental differences are encoded in their weights? In this work, we study the internal representations of GANs. To a human observer, a well-trained

% Yet most work on representation learning focuses on feature learning without even considering multiple objects, 

% ●	Traditional VAEs[15] use “single-object” or “flat” vector representations that fail to capture the compositional structure of natural scenes, i.e. the existence of interchangeable objects with common properties. As a result, “multi-object” or object-centric representations have emerged as a promising approach to scene understanding, improving sample-efficiency and generalization for many downstream applications like relational reasoning and control [5, 20, 3].

% ●	Deep generative models have shown promising results in generating realistic images, but it is still non-trivial to generate images with complicated structures. The main reason is that most of the current generative models fail to explore the structures in the images including spatial layout and semantic relations between objects. 

% Fourth Paragraph model

% intro:

% ●	In this work, we investigate object compositionality for Generative Adversarial Networks (GANs) (Goodfellow et al., 2014) 1 . We investigate a minimal modification to a standard neural network generator that incorporates the right inductive bias and find that it reliably learns to generate images as compositions of objects. Using this general design as a backbone, we then propose two useful extensions that provide a means to incorporate dependencies among objects and background in the generative process. Finally, we demonstrate how one can leverage the learned structured generative process, which is now interpretable and semantically understood, to perform inference and recover individual objects from multi-object images without additional supervision
% ●	In order to formulate the structure (inductive bias) required to achieve object compositionality in neural network generators, we will focus on the corresponding type of invariance that we are interested in. It is concerned with independently varying the different objects that an image is composed of, which requires these to be identified at a representational level and described in a common format.
% ●	and the weights among the generators are shared, such that any acquired knowledge in generating a specific object is transferred across all others. Hence, rather than having to learn about all combinations of objects (including their own variations) that may appear in an image, it suffices to learn about the different variations of each individual object. This greatly simplifies the generative process without losing generality.
% ●	% 
% In order to facilitate relationships of this kind our first extension consists of a relational stage, in which the representation of an object is updated as a function of all others, before each generator proceeds to generate its image.
% ●	Prior works on incorporating inductive biases aimed at object compositionality typically treat an image as a spatial mixture of image patches and utilizes multiple copies of the same function to arrive at a compositional solution.

% ●	In this paper, a sequential scene generation model based on Generative Adversarial Networks is proposed. This model adopts the layered structure modeling for images and generates an image step-by-step starting with the background of the scene and forms the scene progressively by drawing a single foreground object at each step. Finally, it is shown that it resolves the occlusion artifacts of the existing conditional GANs models.
% ●	generating a layered image representation or predicting the depth ordering of the objects in the image 

% ●	In this paper, we aim to teach a machine how to make a pizza by building a generative model that mirrors this step-by-step procedure, To do so, we 
% ●	The proposed model is able to decompose an image into an ordered sequence of layers by applying sequentially in the right order the corresponding removing modules.
% ●	Going beyond food, the concept of “layers” is widespread in digital image editing, where images are composed by combining different layers with different alpha masks. 
% ●	our model can successfully capture the intrinsic structure in the scenes and generate images of complicated scenes accordingly.
% ●	the images with complex relations can be generated effectively and conditionally with the scene configurations appropriately harnessed;
% ●	such that the relation among the objects can be modeled in a flexible way. It therefore not only alleviates the difficulties of training GAN for large-scale images, but facilitates a deeper understanding of the complicated scene configuration.
% ●	highly interpretable and editable structures., refinement

% ●	In this paper, we propose a method for augmenting and training CNNs so that their learned features are compositional. It encourages networks to form representations that disentangle objects from their surroundings and from each other, thereby promoting better generalization

% ●	Our approach compares favorably to state-of-the-art methods in terms of visual fidelity and 3D consistency while generalizing to high spatial resolutions. As we show in our experiments, the learned representations lead to feature activations that are more localized and improve performance over non-compositional baselines in object recognition tasks

% ●	In this paper, we follow a similar philosophy, but focus our attention on the inductive bias of compositionality: the notion that the representation of the whole should be composed of the representation of its parts (we give a precise formal definition of this notion in Sect. 3). Intuitively, encouraging this property during training results in representations that are more robust to re-combination (e.g., when seeing a familiar object in a novel context) and less prone to focusing on discriminative but irrelevant background features. It is also in line with findings from neuroscience that suggest separate processing of figure and ground regions in the visual cortex [16, 32]. 
% ●	In contrast to previous work that designs compositional representations from the ground up [34, 45, 43, 47],

%  Our work serves a complementary purpose in terms of image generation in that regard: while we consider visually simpler scenes, we do not require any extra information about scenes or objects. In the context of representation learning, we are also able to ‘invert’ the learned generative model by leveraging its structure to learn about objects. This sets us firmly apart from these methods and also from standard unstructured GANs that do not rely on conditioning. Indeed, without explicitly considering objects at a representational level (requiring architectural structure), one is unable to recover individual objects in this way. Our approach is different insofar we present a structured generator that facilitates both generation and segmentation of visual scenes that are composed of multiple objects and background, and which is trained purely for generation purposes.
% ●	Our approach is different insofar we present a structured generator that facilitates both generation and segmentation of visual scenes that are composed of multiple objects and background, and which is trained purely for generation purposes

% ●	It incorporates prior knowledge about the compositional nature of human perception to factor interactions between object-pairs and learn efficiently. 
% ●	Common-sense physical reasoning is facilitated by the discovery and representation of objects (a core domain of human cognition (Spelke & Kinzler, 2007)) that serve as primitives of a compositional system. They allow humans to decompose a complex visual scene into distinct parts, describe relations between them and reason about their dynamics as well as the consequences of their interactions (Battaglia et al., 2013; Lake et al., 2016; Ullman et al., 2017). The most successful machine learning approaches to common-sense physical reasoning incorporate such prior knowledge in their design. They maintain explicit object representations,

% ●	We have argued that the ability to discover and describe a scene in terms of objects provides an essential ingredient for common-sense physical reasoning. This is supported by converging evidence from cognitive science and developmental psychology that intuitive physics and reasoning capabilities are built upon the ability to perceive objects and their interactions (Spelke, 1988; Ullman et al., 2017). The fact that young infants already exhibit this ability, may even suggest an innate bias towards compositionality (Lake et al., 2016; Munakata et al., 1997; Spelke & Kinzler, 2007). I  In summary, we believe that our method presents an important step towards learning a more human-like model of the world in a completely unsupervised fashion Current limitations of our approach revolve around grouping and prediction. What aspects of a scene humans group together typically varies as a function of the task in mind. One may perceive a stack of chairs as a whole if the goal is to move them to another room, or as individual chairs if the goal is to count the number of chairs in the stack. In order to facilitate this dynamic grouping one would need to incorporate top-down feedback from an agent into the grouping procedure to deviate from the built-in inductive biases.
% ●	In this paper, we combine the merits of sequential generation with the flexibility of GANs. Our model for sequential generation imbibes a recursive structure that more naturally mimics image composition by inferring three components: appearance, shape, and pose. One closely related work combining recursive structure with GAN is that of Im et al. (2016) but it does not explicitly model object composition and follows a similar paradigm as by Gregor et al. (2015). Another closely related work is that of Kwak & Zhang (2016). It combines recursive structure and alpha blending. However, our work differs in three main ways: (1) We explicitly use a generator for modeling the foreground poses. That provides significant advantage for natural images, as shown by our ablation studies; (2) Our shape generator is separate from the appearance generator. This factored representation allows more flexibility in the generated scenes; (3) Our recursive framework generates subsequent objects conditioned on the current and previous hidden vectors, and previously generated object. This allows for explicit contextual modeling among generated elements in the scene. See Fig. 17 for contextually relevant foregrounds generated for the same background, or Fig. 6 for meaningful placement of two MNIST digits relative to each
% ●	The experimental results suggest that the sequential generation scheme also improves the image quality and the diversity.

% Thirdly, as our results indicate, S2 -GAN allows us to learn RGBD representation in an unsupervised manner. This can be crucial for many robotics and graphics applications. Finally, our Style-GAN can also be thought of as a learned rendering engine which, given any 3D input, allows us to render a corresponding image. 

% ●	Single-object-single-view (SOSV). Many recent breakthroughs in unsupervised representation learning of have come in the form of “disentanglement” models [11, 6, 14] that seek feature-attributelevel understanding by encouraging e.g. independence among latent dimensions. However, most of these models focus on a single view of a single object that has been placed in front of some background (e.g. dSprites, CelebA, 3D Chairs). As a result, they fail to i) generalize to more realistic, multi-object scenes, and ii) accurately capture 3D scene information (e.g. resolve single-view spatial ambiguities and estimate e.g. rotation along the vertical axis). Multi-object-single-view (MOSV). To avoid the additional computational complexities of factorising or segmenting the objects in a scene into explicit multi-object representations, many works have used pre-segmented images [25, 26]. However, this comes at the cost of decreased representational power (good object representation requires good object segmentation [9]) and a reliance on annotated data. In addition, these works struggle in a multi-view scenario where pre-segmented images require consistent multi-frame object registration and tracking, since the segmentation and representation models work independently. More recently, several works [4, 9, 18, 17, 1] have succeeded in approximating the factorized posterior p(z1, z2, ..., zK|x) within the VAE framework

% ●	n internal representation of the scene structure, scene composition
% ●	We develop a GAN model that explicitly encodes this structure. Our proposed model generates images in a recursive fashion: it first generates a background, and then conditioned on the background generates a foreground along with a shape (mask) and a pose (affine transformation) that together define how the background and foreground should be composed to obtain a complete image. Conditioned on this composite image, a second foreground and an associated shape and pose are generated, and so on. As a byproduct in the course of recursive image generation, our approach generates some object-shape foreground-background masks in a completely unsupervised way, without access to any object masks for training. Note that decomposing a scene into foreground-background layers is a classical ill-posed problem in computer vision. By explicitly factorizing appearance and transformation, LR-GAN encodes natural priors about the images that the same foreground can be ‘pasted’ to the different backgrounds,
% ●	As mentioned above, GAN models for synthesizing scenes are capable of encoding hierarchical semantics inside the generative representation, i.e., from layout, object (category), to scene attribute and color scheme. 
% ●	We argue that this notion of consistency can be seen as an inductive bias that improves the efficiency of our learning. Equally, we posit that introducing such a bias towards spatio-temporal consistency into our models should greatly reduce the amount of supervision required for learning. One way of achieving such inductive biases is through model structure.
%  While recent successes in deep learning demonstrate that progress is possible without explicitly imbuing models with interpretable structure (LeCun, Bengio, et al., 2015), recent works show that introducing such structure into deep models can indeed lead to favourable inductive biases improving performance e.g. in convolutional networks (LeCun, Boser, et al., 1989) or in tasks requiring relational reasoning (Santoro et al., 2017). Structure can also make neural networks useful in new contexts by significantly improving generalization, data efficiency (Jacobsen et al., 2016) or extending their capabilities to unstructured inputs (Graves et al., 2016). What inductive biases are good? Minimal sets of principles (bengio)
% ●	Learning decomposed representations of object appearance and position lies at the heart of our model. 

% ●	Stage-I GAN: it sketches the primitive shape and basic colors of the object conditioned on the given text description, and draws the background layout from a random noise vector, yielding a low-resolution image. - Stage-II GAN: it corrects defects in the low-resolution image from Stage-I and completes details of the object by reading the text description again, producing a highresolution photo-realistic image.
% ●	We have investigated the usefulness (and the feasibility) of compositionality at the representational level of objects in GANs through
% ●	And from architectural perspective, can be considered a generalization of the leading StyleGAN model. It also feature multiplicative integration instead of the classic additive update that characterizes the classic transformer used in the NLP community. Qualitative and quantitative experiments show supermesy efficacy, interprtability and disentanglement, support structured scene understanding while generating high quality images. Offering the distribution modelling the, over controlled settings image distribution more accurately. Covering the full-range of the image distribution. 
% ●	This universal design of the MAC cell serves as a structural prior that encourages
% ●	e predicted layout can be used to control generation process.
% ●	Without sacrificing computational or memory efficiency 
% ●	we introduce a generalization of the Transformer  our formulation
% ●	  self-attention mechanism

% ●	In this paper, we explored the effectiveness of image recognition models that are based fully on self-attention. We considered two forms of self-attention: 
% ●	We now formally describe our proposed Attention Augmentation method We therefore do not completely abandon the idea of convolutions, but instead propose to augment convolutions with this selfattention mechanism.
% ●	Next, we explore a different class of operators, which we term

 
% ●	We explore two types 
% ●	 We consider two forms of self-attention.
% ●	 family of operators produce
% ●	 gives the construction significant flexibility
% ●	
% ●	Powerful latent data representations should encode abstract, semantic concepts. Accompanying generative models to decode these rich representations into their varied realizations as data instances, along with learning of the latent representation directly from data represent a coveted guerdon of AI research. 


%  [4, 5, 6, 7, 8]

% As such, the search for expressive, learnable latent encodings along with corresponding generation techniques has been a preoccupation of significant research effort. Examples of data modeling tasks abound. Specifically in this work we consider that of image generation. We are particularly interested in the representation of high-level semantic concepts and hence focus on the depiction of a complex scene x, as illustrated in Fig. 1. Such scenes are composed of a variable number of objects, with individual properties and relations among them. Effective latent representations for these images need flexibility and compositionality. Impressive strides in generative models for images have been made via a number of advances in continuous stochastic latent variable models under the variational auto-encoder (VAE) formalism [1, 2, 3]. We work within this formalism, in which a (conditional) prior p(z|y) controls generation of an output x under condition y via a non-linear mapping pθ(x|z). Recent work (e.g. [3]) has emphasized that the utility of a VAE hinges on its ability to capture useful information in the latent representation z, complementary to that in powerful decoder networks pθ(x|z). 
% ●	On the other hand, renewed interest in programmatic representations in AI have sought modular, generalized, compositional representations for high-level concepts [4, 5, 6, 7, 8]. This line of work uses dynamically programmable networks and has demonstrated impressive results at question answering, graphics-based image rendering, and synthesizing programs for computation or image generation. We build on these approaches to conduct learning of compositional, modular latent representations for scenes. The krux of the problem in learning latent data representations is this dichotomy between powerful decoder networks and the latent encoding. However, structured, complex scenes present an enticing opportunity for learning latent representations. While recent advances in generative modeling have produced exciting progress toward image generation, the successes are largely focused on images of a single object or hand-drawn symbo
% ●	In this work, we propose Self-Attention Generative Adversarial Networks (SAGANs), which introduce a self-attention mechanism into convolutional GANs. The self-attention module is complementary to convolutions and helps with modeling long range, multi-level dependencies across image regions. Armed with self-attention, the generator can draw images in which fine details at every location are carefully coordinated with fine details in distant portions of the image. Moreover, the discriminator can also more accurately enforce complicated geometric constraints on the global image structure. In addition to self-attention, we also incorporate recent insights relating network conditioning to GAN performance. The work by (Odena et al., 2018) showed that well-conditioned generators tend to perform better. We propose enforcing good conditioning of GAN generators using the spectral normalization technique that has previously been applied only to the discriminator (Miyato et al., 2018). We have conducted extensive experiments on the ImageNet dataset to validate the effectiveness of the proposed selfattention mechanism and stabilization techniques. SAGAN significantly outperforms prior work in image synthesis by boosting the best reported Inception score from 36.8 to 52.52 and reducing Frechet Inception distance ´ from 27.62 to 18.65. Visualization of the attention layers shows that the generator leverages neighborhoods that correspond to object shapes rather than local regions of fixed shape. Our code is available at https://github.com/ brain-research/self-attention-gan. 2. 

% ●	The proposed SAGAN generates images by leveraging complementary features in distant portions of the image rather than local regions of fixed shape to generate consistent objects/scenarios. In each row, the first image shows five representative query locations with color coded dots. The other five images are attention maps for those query locations, with corresponding color coded arrows summarizing the most-attended regions

% ●	
% ●	Convolutional generative adversarial networks have demonstrated impressive results in synthesizing high-resolution images [6, 26, 34, 53] from unstructured image collections. However, despite this success, state-of-the-art models struggle to properly disentangle the underlying generative factors including 3D shape and viewpoint. This is in stark contrast to humans who have the remarkable ability to reason about the 3D structure of the world and imagine objects from novel viewpoints.

% ●	Generative Adversarial Networks (GANs) can produce images of remarkable complexity and realism but are generally structured to sample from a single latent source ignoring the 

% ●	One open challenge widely observed in global image-level generation methods is the difficulty of generating small objects and detailed local texture. To tackle this issue a local context, and correspondingly design a local class-specific generative network with semantic maps as a guidance
%  ●	
% the need for a better understanding of “what makes them tick” and  

% ●	S a longstanding and fundamental challenge in computer vision research, realistic image synthesis has been attracting increasing attention since the advent of deep neural networks (DNNs). An important driving factor is the data constraint in DNNs training, where synthetic data is much cheaper, faster and more scalable as compared to the traditional manual collection approach. In recent years, the advance of generative adversarial networks (GANs) [1] opens a new door for image synthesis by iterative adversarial learning between a generator and a discriminator. Quite a number of GAN-based image synthesis systems have been reported which generate new images by direct image generation from random noises [2], image-to-image translation [3], [4] and image composition [5], [6], [7]. 

% On the other hand, existing image synthesis systems are still facing two common constraints. First, most existing systems only strive for synthesis realism in either appearance domain or geometry domain instead of both domains. Second, many existing systems tend to sacrifice image details and resolutions and even semantics of the image contents to synthesize realistic images. Specifically, the direct generation based methods [1], [2] cannot guarantee the accurate image labels or annotations, thus the synthesized images often lack sufficient semantic integrity for the training of deep models. The image translation based methods [3], [4] only focuses on the synthesis realism in appearance domain with some extend of decreasing in image resolution. The composition based methods [5], [7] can generate labeled or annotated images of high-resolution, but it usually focuses on synthesis realism in geometric domain and can only deal with a single foreground object.

% ●	**** Generative Adversarial Networks (GANs) [15] have significantly advanced image synthesis in recent years. The rationale behind GANs is to learn the mapping from a latent distribution to the real data through adversarial training. After learning such a non-linear mapping, GAN is capable of producing photo-realistic images from randomly sampled latent codes.

% Taking face synthesis as an example, when sampling a latent code to produce an image, how the code is able to determine various semantic attributes (e.g., gender and age) of the output face, and how these attributes are entangled with each other? hesis quality of GANs [40, 28, 21, 8, 22], however, few efforts have been made on studying what a GAN actually learns with respect to the latent space. Radford et al. [31] first observes the vector arithmetic property in the latent space. A recent work [4] further shows that some units from intermediate layers of the GAN generator are specialized to synthesize certain visual concepts, such as sofa and TV for living room generation. Even so, there lacks enough understanding of how GAN connects the latent space and the image semantic space, as well as how the latent code can be used for image editing.

% ●	One of the unsolved key challenges in machine learning is unsupervised learning of structured representation for a visual scene containing many objects with occlusion, partial observability, and complex background. When properly decomposed into meaningful abstract entities such as objects and spaces, this structured representation brings many advantages of abstract (symbolic) representation to areas where contemporary deep learning approaches with a global continuous vector representation of a scene have not been successful. For example, a structured representation may improve sample efficiency for downstream tasks such as a deep reinforcement learning agent (Mnih et al., 2013). It may also enable visual variable binding (Sun, 1992) for reasoning and causal inference over the relationships between the objects and agents in a scene. Structured representations also provide composability and transferability for better generalization.

% ●	. While several recent papers (Bau et al., 2019; Voynov & Babenko, 2019; Yang et al., 2019; Karras et al., 2019; Jahanian et al., 2020; Plumerault et al., 2020) address the interpretability of GANs, this research area is still in its preliminary stage. An active line of study on GANs interpretability investigates the structure of their latent spaces. Namely,  At the moment, prior works have provided enough evidence that a wide range of such directions exists. Some of them induce domainagnostic transformations, like zooming or translation (Jahanian et al., 2020; Plumerault et al., 2020), while others correspond to domain-specific transformations, e.g., adding smile or glasses on face images (Radford et al., 2015).
% ●	The ability to produce high-quality, controllable images has made GANs an increasingly attractive alternative to the traditional graphics pipeline for content generation. However, most work focuses on property disentanglement, such as shape, pose and appearance, without considering the compositionality of the images, i.e., scenes being made up of multiple objects. Therefore, they do not offer control over individual objects in a way that respects the interaction of objects, such as consistent lighting and shadows. This is a major limitation of current image generative models, compared to the graphics pipeline,

% ●	Despite the success of Generative Adversarial Networks (GANs) in image synthesis, there lacks enough understanding on what generative models have learned inside the deep generative representations and how photo-realistic images are able to be composed of the layer-wise stochasticity introduced in recent GANs. In this work, we show that highlystructured semantic hierarchy emerges as variation factors from synthesizing scenes from the generative representations in state-of-the-art GAN models, like StyleGAN and BigGAN
% ●	
% ●	Deep generative models of images have received considerable attention following the seminal works on variational autoencoders (Kingma & Welling, 2014) and generative adversarial networks (Goodfellow et al., 2014). The vast majority of such models use a monolithic, unstructured latent space, that represents an entire scene in an unfactored fashion. Recently, however, several generative models have emerged that use an object-centric representation instead.

% ●	
% ●	
% Here, we use a latent regressor to probe the latent space of a pretrained GAN, allowing us to uncover and manipulate the concepts that GANs learn about the world in an unsupervised manner.

% Deep generative models have led to remarkable breakthroughs in learning hierarchical representations of images and decoding them back to images [Goodfellow et al., 2014]. 
% However, the obtained representation is often limited to a single object, hard to interpret, and missing the complex 3D structure behind visual input. As a result, these deep generative models cannot support manipulation tasks such as moving an object around as in Fig. 1. On the other hand, computer graphics engines use a predefined, structured, and disentangled input (e.g., graphics code), often intuitive for scene manipulation. However, it is in general intractable to infer the graphics code from an input image.

% ●	object-based, interpretable scene representation into a deep generative model

% ●	Existing work typically focuses on improving the synthesis quality of GANs [40, 28, 21, 8, 22], however, few efforts have been made on studying what a GAN actually learns with respect to the latent space. Radford et al. [31] first observes the vector arithmetic property in the latent space. A recent work [4] further shows that some units from intermediate layers of the GAN generator are specialized to synthesize certain visual concepts, such as sofa and TV for living room generation. Even so, there lacks enough understanding of how GAN connects the latent space and the image semantic space, as well as how the latent code can be used for image editing.

% ●	GAN-based Image Synthesis: Generative Adversarial Networks (GANs) [24] have been shown to allow for photorealistic image synthesis at resolutions of 10242 pixels and beyond [6, 14, 15, 38, 39]. To gain better control over the synthesis process, many works investigate how factors of variation can be disentangled without explicit supervision. They either modify the training objective [9, 39, 70] or network architecture [38], or investigate latent spaces of well-engineered and pre-trained generative models [1, 16, 23, 26, 33, 77, 95]. All of these works, however, do not explicitly model the compositional nature of scenes. Recent works therefore investigate how the synthesis process can be controlled at the object-level [3,4,7,18,19,25,44,85,89]. While achieving photorealistic results, all aforementioned works model the image formation process in 2D, ignoring the three-dimensional structure of our world. In this work, we advocate to model the formation process directly in 3D for better disentanglement and more controllable synthesis.

% ●	Deep generative models allow for photorealistic image synthesis at high resolutions. But for many applications, this is not enough: content creation also needs to be controllable. While several recent works investigate how to disentangle underlying factors of variation in the data, most of them operate in 2D and hence ignore that our world is three-dimensional. Further, only few works consider the compositional nature of scenes. Our key hypothesis is that incorporating a compositional 3D scene representation into the generative model leads to more controllable image synthesis.

% ●	The ability to generate and manipulate photorealistic image content is a long-standing goal of computer vision and graphics. Modern computer graphics techniques achieve impressive results and are industry standard in gaming and movie productions. However, they are very hardware expensive and require substantial human labor for 3D content creation and arrangement.  They are able to synthesize photorealistic images at resolutions of 10242 pixels and beyond [6,14,15,38,39]. Despite these successes, synthesizing realistic 2D images is not the only aspect required in applications of generative models. The generation process should also be controllable in a simple and consistent manner. To this end, many works [9, 38, 42, 43, 47, 53, 70, 73, 96] investigate how disentangled representations can be learned from data without explicit supervision. 

% in the 2D domain, ignoring that our world is three-dimensional.  (Fig. 2) and control mechanisms are not built-in, but need to be discovered in the latent space a posteriori. These properties, however, are crucial for successful applications, e.g. a movie production where complex object trajectories

% ●	most existing approaches do not specifically model objects and their relations in images and thus have difficulties in generating complex scenes such as those in the COCO dataset [15]. o make them look realistic (see the middle row of Fig. 1). In this study, we aim to generate high-quality complex images with semantically meaningful layout and realistic objects. To this end, we propose a novel

% ********* (Burgess et al., 2019; van Steenkiste et al., 2018; Eslami et al., 2016) we maintain that discovery of objects in a scene should be considered a crucial aspect of representation learning, rather than treated as a separate problem

% ●	According to paper complex eval “exploiting scene compositionality in the generator helps improve generalization.” the individual quality of the generated objects generally suffers from missing high frequency details, especially for objects belonging to the long tail classes of the dataset. T
% ●	
% ●	Traditional VAEs[15] use “single-object” or “flat” vector representations that fail to capture the compositional structure of natural scenes, i.e. the existence of interchangeable objects with common properties, doesn’t explicitly account for
% ●	Deep generative models [Goodfellow et al., 2014] have been used to synthesize realistic images and learn rich internal representations. Representations learned by these methods are typically hard for humans to interpret and understand, often ignoring the 3D nature of our visual world. M
% ●	

% ●	we propose to employ multiple latent codes and compose their corresponding feature maps at some intermediate layer of the generator. Utilizing multiple latent codes allows the generator to recover the target image using all the possible composition knowledge learned in the deep generative representation
% ●	In this paper, we propose the Self-Attention Generative Adversarial Network (SAGAN) which allows attention-driven, long-range dependency modeling for image generation tasks. Traditional convolutional GANs generate high-resolution details as a function of only spatially local points in lower-resolution feature maps. In SAGAN, details can be generated using cues from all feature locations. Moreover, the discriminator can check that highly detailed features in distant portions of the image are consistent with each other. Furthermore, recent work has shown that generator conditioning affects GAN performance.
% ●	

% ●	In this work, we study the internal representations of GANs. To a human observer, a well-trained GAN appears to have learned facts about the objects in the image: for example, a door can appear on a building but not on a tree. We wish to understand how a GAN represents such a structure. Do the objects emerge as pure pixel patterns without any explicit representation of objects such as doors and trees, or does the GAN contain internal variables that correspond to the objects that humans perceive? If the GAN does contain variables for doors and trees, do those variables cause the generation of those objects, or do they merely correlate? How are relationships between objects represented?
% ●	The new architecture leads to an automatically learned, unsupervised separation of high-level attributes (e.g., pose and identity when trained on human faces) and stochastic variation in the generated images (e.g., freckles, hair), and it enables intuitive, scale-specific control of the synthesis.

% ******* ●	A compositional representation consists of components that can be recombined, and such recombination underlies generalization. For example, consider a pink elephant. With a representation that composes color and object independently, imagining a pink elephant is trivial. However, a pink elephant may not be within the scope of a representation that mixes color and object. Compositionality comes in a variety of flavors, including feature compositionality (e.g. pink elephant), multi-object compositionality (e.g. elephant next to a penguin), and relational compositionality (e.g. the smallest elephant). In this paper we will focus on feature compositionality - within reach of Representations with feature compositionality are sometimes referred to as “disentangled” representations [Bengio et al., 2013]. However, there is as yet no consensus on the definition

% ●	Combined with noise injected directly into the network, this architectural change leads to automatic, unsupervised separation of high-level attributes (e.g., pose, identity) from stochastic variation (e.g., freckles, hair) in the generated images, and enables intuitive scale-specific mixing and interpolation operations



% ●	
% ●	step towards robust compositional visual representation learning
% ●	This paper studies the interesting but difficult problem of generating physically plausible scenes and videos which contain multiple objects that interact with each other. The generative model is formulated based on GAN by extending a 2D variant of BlockGAN with a relational layer. The proposed model includes a correction network to model object interactions and a structural loss function to evaluate the object poses.
% ●	 It improves on past work by using a relational architecture for generating the objects, which allows the network to model dependencies between objects. 


% ●	In this work, we show that highly-structured semantic hierarchy emerges as variation factors from synthesizing scenes from the generative representations in state-of-the-art GAN models, like StyleGAN and BigGAN. the early layers tend to determine the spatial layout and configuration, the middle layers control the categorical objects, and the later layers finally render the scene attributes as well as color scheme. Identifying such a set of manipulatable latent variation factors facilitates semantic scene manipulation

% ●	highly-structured semantic hierarchy emerges from the deep generative representations with layer-wise stochasticity trained for synthesizing scenes, even without any external supervision.

% It is postulated that knowledge about the generative process exposes important factors of variation in the environment

% positions/locations

% it is important that the structure of the generative model closely resembles the underlying generative process.
% , represenation 

% capacities for reasoning, imagining, planning, and learning 
% object-oriented representation for visual scenes serves as the basis  reasoning, imagining, learning and planning.

% Human intelligence is object-oriented. Infants begin parsing the world into distinct objects within their first months of life [13], and our sophisticated capacities for reasoning, imagining, planning, and learning depend crucially on our representation of the world as dynamic objects and their relations. 

% This core object knowledge was learned through evolution and experience, and is very useful. It can be shared across object instances,provides a means for some properties of the world to be highly dependent and others to be relatively independent, and allows objects to be composed to form abstractions and hierarchies whose wholes are greater than the sums of their parts. 

% Representing the world as objects is core to human intelligence. It is the basis of people’s sophisticated capacities for reasoning, imagining, planning, and learning.
% the model can learn interpretable representations of visual scenes that disentangle objects and their properties.

% As a result, “multi-object” or object-centric representations have emerged as a promising approach to scene understanding, improving sample-efficiency and generalization for many downstream applications like relational reasoning and control [5, 20, 3].

% The human percept of a visual scene is highly structured. Scenes naturally decompose into objects that are arranged in space, have visual and physical properties, and are in functional relationships with each other. 
% scene elements 

% Realistic visual scenes contain rich structure, which humans effortlessly exploit to reason effectively and intelligently. In particular, object perception, the ability to perceive and represent individual objects, is considered a fundamental cognitive ability that allows us to understand – and efficiently interact with – the world as perceived through our senses [Johnson, 2018, Green and Quilty-Dunn, 2017]. 

% Natural scenes are comprised of disparate parts and objects that humans can easily segment and interchange 

% Human perception is structured around objects which form the basis for our higher-level cognition and impressive systematic generalization abilities.


% Complicated scene images contain varied visual elements, compositional visual concepts, and complicated relations between objects. 

% Humans naturally perceive the world as being structured into different objects, their properties and relation to each other.

% This rich structure is crucial for many real-world tasks such as manipulating objects or driving a car, where awareness of different objects and their features is required.

% slotatt:
% Object-centric representations have the potential to improve sample efficiency and generalization of machine learning algorithms across a range of application domains, such as visual reasoning [1], modeling of structured environments [2], multi-agent modeling [3–5], and simulation of interacting physical systems [6–8]. 

% Probabilistic generative models aim to recover the process with which the observed data was generated

% A promising, but under-explored, inductive bias in deep generative models of images is compositionality at the representational level of objects, which accounts for the compositional nature of the visual world and our perception thereof (Spelke  Kinzler, 2007; Battaglia et al., 2013)

% It allows a generative model to describe a scene as a composition of objects, thereby ‘disentangling’ visual information that can be processed largely independently of one another. By explicitly accounting for object compositionality one imposes an invariance that simplifies the generative process, and potentially allows one to (more efficiently) learn a more accurate generative model of images. Moreover, by explicitly considering individual objects at a representational level, (posterior) inference in the learned generative model allows one to recover corresponding object representations that are desirable for many ‘down-stream’ learning tasks (Santoro et al., 2017; Janner et al., 2019)

% Compositional reasoning in terms of objects, relations, and actions is a central ability in human cognition (Spelke & Kinzler, 2007). These structured neural models greatly facilitate predicting physical dynamics and the consequences of actions, and provide a strong inductive bias for generalization to novel environment situations, allowing models to answer counterfactual questions A structured understanding of our world in terms of objects, relations, and hierarchies is an important component of human cognition. 

% entire scenes built from them Moreover, we can decompose a novel image in terms of the objects it shows, identifying their locations, distances and extents, and even reasoning about occluded parts.
% Images are composed of several different objects forming a hierarchical structure with various styles and shapes.


% Humans typically interpret a scene in a hierarchy of semantics, from its layout, underlying objects, to the detailed attributes and the color scheme. 

% Deep generative models seek to recover the process with which the observed data was generated.  However, a bias to account for the compositional way in which humans structure a visual scene in terms of objects has frequently been overlooked. 

% ●	They may be used to synthesize new samples or to subsequently extract representations.
%  Successful approaches in the domain of images are driven by several core inductive biases. 

% Modeling compositionality in natural images is a challenging problem due to the complex interactions among different objects with respect to relative scaling, spatial layout, occlusion or viewpoint transformation. 


 
 % Recent work using spatial transformer networks [11] within a GAN framework [16] decomposes this problem by operating in a geometric warp parameter space to find a geometric modification for a foreground object. However, this approach is only limited to a fixed background and does not consider more complex interactions in the real world
 
% ●	One fundamental limitation of these methods is that they attempt to generate images without taking into account that images are 2D projections of a 3D visual world, which has a lot of structures in it. This manifests as structure in the 2D images that capture this world. One example of this structure is that images tend to have a background, and foreground objects are placed in this background in contextually relevant ways.
 
%  In this work, we investigate object compositionality as an inductive bias for Generative Adversarial Networks (GANs). it reliably learns to generate images as compositions of objects. Using this general design as a backbone, we then propose two useful extensions to incorporate dependencies among objects and background. We extensively evaluate our approach on several multi-object image datasets and highlight the merits of incorporating structure for representation learning purposes. In particular, we find that our structured GANs are better at generating multi-object images that are more faithful to the reference distribution. More so, we demonstrate how, by leveraging the structure of the learned generative process, one can ‘invert’ the learned generative model to perform unsupervised instance segmentation.

% ●	Learning object-centric representations of complex scenes is a promising step towards enabling efficient abstract reasoning from low-level perceptual features. In this paper, we present the Slot Attention module, an architectural component that interfaces with perceptual representations such as the output of a convolutional neural network and produces a set of task-dependent abstract representations which we call slots. These slots are exchangeable and can bind to any object in the input by specializing through a competitive procedure over multiple rounds of attention. We empirically demonstrate that Slot Attention can extract object-centric representations that enable generalization to unseen compositions when trained on unsupervised object discovery and supervised property prediction tasks.
% ●	The ability to reason about the relations between entities and their properties is central to generally intelligent behavior (Figure 1) [18, 15]. Other approaches, such as those based on statistical learning, build representations from raw data and often generalize across diverse and noisy conditions [25]. However, a number of these approaches, such as deep learning, often struggle in data-poor problems where the underlying structure is characterized by sparse but complex relations  specify any particular form or semantics of the internal object representations This demonstrates the RN’s rich capacity for structured reasoning even with unstructured inputs and outputs.  Future work should apply RNs to a variety of problems that can benefit from structure learning and exploitation, such as rich scene understanding in RL agents, modeling social networks, and abstract problem solving.

% Generative models, as an analysis-by-synthesis process, should encompass the following three core components: 1) the generation process that composes the scene; 2) what are the primitive visual elements and how are they composed; 3) the rendering of abstract concepts into their pixel-level realizations

%  This phenomenon which we refer to as perceptual grouping is also known as amodal perception in psychology. It occurs effortlessly and includes a segmentation of the visual input, such as that shown in in Figure 1. This grouping also applies analogously to other modalities, for example in solving the cocktail party problem (audio) or when separating the sensation of a grasped object from the sensation of fingers touching each other (tactile). Even more abstract features such as object class, color, position, and velocity are naturally grouped together with the inputs to form coherent objects. 
 
% ●	Obtaining object-centric representations from raw perceptual input, such as an image or a video, is challenging and often requires either supervision [1, 3, 9, 10] or task-specific architectures [2, 11]. As a result, the step of learning an object-centric representation is often skipped entirely. Instead, models are typically trained to operate on a structured representation of the environment that is obtained, for example, from the internal representation of a simulator [6, 8] or of a game engine [4, 5].

% ●	Probabilistic generative models aim to recover the process with which the observed data was generated. It is postulated that knowledge about the generative process exposes important factors of variation in the environment (modeled by latent variables) that may subsequently be obtained using an appropriate posterior inference procedure. Hence, in order to use generative models for representation learning, it is important that the structure of the generative model closely resembles the underlying generative process. Deep generative models of images rely on the expressiveness of neural networks to learn the generative process directly from data
% ●	Their structure is determined by the inductive bias of the neural network, which steers it to organize its computation in a way that allows salient features to be recovered and ultimately captured in a representation (Kingma & Welling, 2014; Dinh et al., 2017; Donahue et al., 2017; Dumoulin et al., 2017). Recently, it was shown that independent factors of variation, such as pose and lighting of human faces may be recovered in this way (Chen et al., 2016; Higgins et al., 2017). . 







% ●	

% Here the underlying objects refer to the set of objects most relevant to a specific category. This section shows that GAN composes a scene over the layers in a similar way with human perception.
% ●	Images are composed of several different objects forming a hierarchical structure with various styles and shapes. Deep learning models are used to disentangle those complex underlying patterns (Reed et al. 2014)(Wang and Gupta 2016), build distributed feature representations (Hinton and Salakhutdinov 2006), and solve classification (Krizhevsky et al. 2012) and gener

% ●	As humans, we naturally understand the world in terms of objects. We know the typical appearance of many types of object, and can imagine new instances of them—or indeed, entire scenes built from them. Moreover, we can decompose a novel image in terms of the objects it shows, identifying their locations, distances and extents, and even reasoning about occluded parts.

% ●	 This ability serves as a core motivation behind a range of recent works that aim at enriching machine learning models with the ability to disentangle scenes into objects, their properties, and relations between them (Chang et al., 2016; Battaglia et al., 2016; Watters et al., 2017; van Steenkiste et al., 2018; Kipf et al., 2018; Sun et al., 2018; 2019b; Xu et al., 2019). These structured neural models greatly facilitate predicting physical dynamics and the consequences of actions, and provide a strong inductive bias for generalization to novel environment situations, allowing models to answer counterfactual questions such as “What would happen if I pushed this block instead of pulling it?”. A structured understanding of our world in terms of objects, relations, and hierarchies is an important component of human cognition. 






% ●	In this paper, we show the emergence of highly-structured variation factors inside the deep generative representations learned by GANs with layer-wise stochasticity. In particular, the GAN model spontaneously learns to set up layout at early layers, generate categorical objects at middle layers, and render scene attribute and color scheme at later layers when trained to synthesize scenes. A re-scoring method is proposed to quantitatively identify the manipulatable semantic concepts within a well-trained model, enabling photorealistic scene manipulation. We will explore to extend this manipulation capability of GANs for real image editing in future work.

% ●	

% or treats segmentation as an (often supervised) preprocessing step. Instead, we argue for the importance of learning to segment and represent objects jointly. We demonstrate that, starting from the simple assumption that a scene is composed of multiple entities, it is possible to learn to segment images into interpretable objects with disentangled representations. Our method learns – without supervision – to inpaint occluded parts, and extrapolates to scenes with more objects and to unseen objects with novel feature combinations. We also show that, due to the use of iterative variational inference, our system is able to learn multi-modal posteriors for ambiguous inputs and extends naturally to sequences

% ●	Our second source of motivation is the role of mental imagery and simulation in human cognition [18]. Mental imagery is believed to play an important role in planning and decision making. The level of detail and completeness of mental imagery is a matter of debate, but its role in human intelligence suggests that the ability to synthesize photorealistic images may support the development of artificial intelligent systems [24].

% ●	Researchers have developed scene representations that take object-part hierarchy and inter-object relations into account. In particular, scene graphs [28] are a representation that simultaneously captures objects and their relations within a single image. While most related works on inferring scene graph representations from visual data require fine-grained annotations, several works have studied inferring objects and their relations from videos without supervision [50, 43, 53]. These models have the most similar setup as ours, but all focus on 2D pixel-level segmentation only. Several recent papers have explored building 3D, object-centric scene representations from raw visual observations. However, none of them have yet attempted to model the hierarchy between objects and parts or the relations between multiple scene components 
% ●	A fundamental problem of vision is how to deal with the enormous complexity of images and visual scenes 1 . The total number of possible images is almost infinitely large [8]. The number of objects is also huge and has been estimated at around 30,000 [2]. How can a biological, or artificial, vision system deal with this complexity? For example, considering the enormous input space of images and output space of objects, how can humans interpret images in less than 150 msec [16]? There are three main issues involved. Firstly, how can a visual system be designed so that it can efficiently represent large classes of objects, including their parts and subparts? Secondly, how can the visual system be designed so that it can rapidly infer which object, or objects, are present in an input image and the positions of their subparts? And, thirdly, how can this representation be learnt in an unsupervised, or weakly supervised fashion? In short, what visual architectures enable us to address these three issues? Many considerations suggest that visual architectures should be hierarchical. The structure of mammalian visual systems is hierarchical with the lower levels (e.g., in areas V1 and V2) tuned to small image features while the higher levels (i.e. in area IT) are tuned to objects 2 . Moreover, as appreciated by pioneers such as Fukushima [5], hierarchical architectures lend themselves naturally to efficient representations of objects in terms of parts and subparts which can be shared between many objects. Hierarchical architectures also lead to efficient learning algorithms as illustrated by deep belief learning and others [7]. There are many varieties of hierarchical models which differ in details of their representations and their learning and inference algorithms [14, 7, 15, 1, 13, 18, 10, 3, 9]. But, to the best of our knowledge, there has been no detailed study of their complexity properties


% ●	THE ability to learn abstract representations that support transfer to novel but related tasks lies at the core of many problems in computer vision, natural language processing, cognitive science, and machine learning. In typical applications of machine classification algorithms today, learning a new concept requires tens, hundreds, or thousands of training examples. For human learners, however, just one or a few examples are often sufficient to grasp a new category and make meaningful generalizations to novel instances [15], [25], [31], [44]. Clearly, this requires very strong but also appropriately tuned inductive biases. 
% ●	However, these approaches ignore one of the most basic underlying principles of image formation. Images are a product of two separate phenomena: Structure: this encodes the underlying geometry of the scene. It refers to the underlying mesh, voxel representation etc. Style: this encodes the texture on the objects and the illumination.


% ●	Human intelligence is object-oriented. Infants begin parsing the world into distinct objects within their first months of life [13], and our sophisticated capacities for reasoning, imagining, planning, and learning depend crucially on our representation of the world as dynamic objects and their relations. 
% Though the human notion of an object is rich, and exists in an even richer continuum of non-solids, non-rigids, object parts, and multi-object configurations, here we use the term “object” simply as a discrete visual entity localized in space. 
% Many important domains of artificial intelligence use representations of objects that were chosen ahead of time by humans, based on subjective knowledge of what constitutes an object (e.g. patches in images that can be categorized, or geometric meshes for physical control). This core object knowledge was learned through evolution and experience, and is very useful. It can be shared across object instances, provides a means for some properties of the world to be highly dependent and others to be relatively independent, and allows objects to be composed to form abstractions and hierarchies whose wholes are greater than the sums of their parts. Given the importance of such representations, and the high cost of manually translating it from the engineer’s mind into AI datasets and architectures, this work asks: How can an artificial system learn, without supervision, an object-based representation? Our contributions are: (1) a probabilistic model that can learn object-based representations from data, (2) a visual attention mechanism for inferring a sparse set of objects from images.

% ●	
% ●	factorized object representations for foreground objects while also decomposing background segments of complex morphology




% ●	Representing the world as objects is core to human intelligence. It is the basis of people’s sophisticated capacities for reasoning, imagining, planning, and learning. Artificial intelligence typically assumes human-defined representations of objects, and little work has explored how object-based representations can arise through unsupervised learning. Here we present an approach for learning probabilistic, object-based representations from data, called the “multi-entity variational autoencoder” (MVAE), whose prior and posterior distributions are defined over a set of random vectors. We demonstrate that the model can learn interpretable representations of visual scenes that disentangle objects and their properties.

% ●	David Marr has defined vision as the process of discovering from images what is present in the world, and where it is [15]. The combination of what and where captures the essence of an image at the semantic level and therefore, also plays a crucial role when defining the desired output of image synthesis tools following the general philosophy of introducing compositionality into representation.

% ●	

% ●	Compositionality (e.g. [10]), which serves as a foundation for this contribution, is a general principle in cognition and can be especially observed in human vision [3]. Perception has a high tendency to represent complex entities by means of comparably few, simple, and widely usable parts together with relations between them. In contrast to modeling an object directly based on a constellation of its parts (e.g. [8]), the compositional approach learns intermediate groupings of parts. As a consequence, compositions bridge the semantic gap between low level features and high level object recognition by establishing intermediate hidden layer representations. In conclusion, compositions model category-distinctive subregions of an object, which show small intra-category variations compared to the whole object

% ●	With this relational approach, it can composite visual elements into higher-level entities in a more efficient manner that benefits semantic inference.

% This problem can be also seen as perceptual grouping, which involves modelling pixels as spatial mixtures of entities. 
% ●	Science fiction has long dreamed of virtual realities filled of synthetic content as rich as, or richer, than the real world (e.g., The Matrix, Ready Player One). How close are we to this dream? Traditional computer graphics can render photorealistic 3D scenes, but cannot automatically generate detailed content. Generative models like GANs, in contrast, can create content from scratch, but we do not currently have tools for navigating the generated scenes in the same kind of way as you can walk through and interact with a 3D game engine.

% ●	This question is connected to central problems in computer graphics and artificial intelligence. First, consider the problem of photorealism in computer graphics. A system that synthesizes photorealistic images from semantic layouts would in effect function as a kind of rendering engine that bypasses the laborious specification of detailed threedimensional geometry and surface reflectance distributions, and avoids computationally intensive light transport simulation [33]. A direct synthesis approach could not immediately replace modern rendering engines, but would indicate that an alternative route to photorealism may be viable and could some day complement existing computer graphics techniques.

% Meanwhile, given a scene image, we are able to extract multiple levels of attributes, as shown in Fig.2. As a comparison, generative models such as GANs follow a completely end-to-end training manner for synthesizing scenes, without any prior knowledge about the drawing techniques and relevant concepts. Even so, the trained GANs are able to produce photo-realistic scenes, which makes us wonder if the GANs have mastered any human-understandable drawing knowledge as well as the variation factors of scenes spontaneously.

% Artificial systems that interpret images in this way are desirable, as accurate detection of objects and inference of their attributes is thought to be fundamental for many problems of interest. Consider a robot whose task is to clear a table after dinner. To plan its actions it will need to determine which objects are present, what classes they belong to and where each one is located on the table. 

% The notion of using structured models for image understanding has a long history (e.g., ‘vision as inverse graphics’ [4]), however in practice it has been difficult to define models that are: (a) expressive enough to capture the complexity of natural scenes, and (b) amenable to tractable inference. Meanwhile, advances in deep learning have shown how neural networks can be used to make sophisticated predictions from images using little interpretable structure (e.g., [10]).

% ●	Natural scenes are comprised of disparate parts and objects that humans can easily segment and interchange (Biederman, 1987). 


% ●	 attends to scene elements
% ●	

% ●	The visual world we sense, interpret and interact everyday is a complex composition of interleaved physical entities. % Therefore, it is a very challenging task to generate vivid scenes of similar complexity using computers. 


% stimulating facilitating  problem solving, and conceptual understanding.

% Sketching is a tool that supports the tacit, complex cognitive processes involved in sense-making, creative discovery, and problem solving.

% important aspects of sketching that facilitate design processes.
% empirical
% inspection and thus perception, rather than to give simultaneous incentives for perception. Second, the role of perception is to stimulate functional thoughts

% intermedia represetnation reflect the way we actually think through problems and provide openings for the new and unforeseen
% allows us for further revaluation 
% aid to short-term memory, sketches are not just about lightening cognitive load
% support radical restructuring of percepts and concepts, stimulating new analogies and leading the way to innovation and invention.



% Rough outlines are gradually replaced by precise forms, lines are sharpened, darkened or erased, shapes are altered, and the final picture emerges.

% a blank canvas that is being filled 
% initiating from a blank 

% cis a form of visual expression

% visual art 

% reflect

% Human-drawn sketches reflect people’s abstract expression of objects. They are highly concise yet expressive: usually several lines can reflect the important morphological features of an object, and even imply more semantic-level information


% A person asked to draw, paint or otherwise recreate a visual scene will naturally do so in a sequential, iterative fashion, reassessing their hand work after each modification. 
% Rough outlines are gradually replaced by precise forms, lines are sharpened, darkened or erased, shapes are altered, and the final picture emerges.

% Our main idea resembles how a landscape painter would first sketch out the overall structure, e.g. first a background such as mountain ranges or rivers, and later embellish the scene gradually with other elements to populate the scene, e.g. foreground instances such as trees and animals. 

% Like a painter that first draws a rough sketch and only then fills in the details. 


% drawing iterative process of refinement create expression cognitive process underlying starting from rough sketches effective drawing, require planning global to details

% Imagine an artist drawing a picture of the living room. The very first step, before drawing every single object, is to choose a perspective and set up the layout of the room. After the spatial structure is set, the next step is to add objects that typically occur in a living room, such as a sofa and TV. Finally, the artist will refine the details of the picture with specified decoration styles, e.g., warm or cold, natural lighting or indoor lighting. The above process reflects how a human draws a scene by interpreting it from multiple abstraction levels. 

% conceptual understanding of the the object  or of a simpl
% conceptions


% In (realistic) painting, a common strategy is to produce images by lightweight rough initial sketch (global planning), so to make sure the overall layout/arrangement and relations between different objects make sense, then painting and refining the details. (Drew paper + general)

% It’s true in fact for most creative tasks, even when one writes a new article/text, or an agent that needs to execute some task in RL, it’s a common and useful strategy to have a global plan first, then focus on the details.

% Artistic development creative process, 
% stages, phases, , sketching, 
% rough outline deleanting the high level structure 
% Second Paragraph deep learning models in contrast. 
% People do different parts but not altogether
% First Paragraph Drawing sketching

% ●	Atiosit generate scenes whether through drawing or computer graphics they use structured approach to generate the scene
% ●	In (realistic) painting, a common strategy is to produce images by lightweight rough initial sketch (global planning), so to make sure the overall layout/arrangement and relations between different objects make sense, then painting and refining the details. (Drew paper + general)
% ●	

% First Paragraph Drawing sketching

% A skilled painter could draw images that depict urban scenes that conform to these layouts. Highly trained craftsmen can even create paintings that approach photorealism [20]. Can we train computational models that have this ability? Given a semantic layout of a novel scene, can an artificial system synthesize an image that depicts this scene and looks like a photograph?

% ●	Human-drawn sketches reflect people’s abstract expression of objects. They are highly concise yet expressive: usually several lines can reflect the important morphological features of an object, and even imply more semantic-level information.

% ●	Understanding how to learn powerful representations from complex distributions is the intriguing goal behind adversarial training on image data. While recent advances have enabled us to generate high-resolution images with Generative Adversarial Networks (GANs), currently most GAN models still focus on modeling images that either contain only one centralized object (e.g. faces (CelebA), objects (ImageNet), birds (CUB-200), flowers (Oxford-102), etc.) or on images from one specific domain (e.g. LSUN bedrooms, LSUN churches, etc.). This means that, overall, the variance between images used for training GANs tends to be low (Raj et al., 2017). However, many real-life images contain multiple distinct objects at different locations within the image and with different relations to each other. This is for example visible in the MS-COCO data set (Lin et al., 2014), which consists of images of different objects at different locations within one image. In order to model images with these complex relationships, we need models that can model images containing multiple objects at distinct locations. 

% ●	In particular, GAN constructs the spatial layout at the early stage, synthesizes category-specified objects at the middle stage, and renders the scene attribute and color scheme at the later stage.

% ●	variants could include layers or successively more abstract information regarding image content. We proposed a novel programmatic approach to constructing priors for generative modeling of complex scenes. A set of modular components can be combined to represent complex abstract concepts. Individual components represent base concepts such as a sphere, or the material property shiny. These are combined via aggregation operators that allow for modification or interactions between components. We demonstrated that these priors can be used to model the variability and compositional aspects of complex images consisting of multiple entities with different properties, outperforming related methods that do not model scene structure.

% ●	Coupling the high-fidelity generation capabilities of label-conditional image synthesis methods with the flexibility of unconditional generative models, we propose a semantic bottleneck GAN model for unconditional synthesis of complex scenes. We assume pixel-wise segmentation labels are available during training and use them to learn the scene structure. During inference, our model first synthesizes a realistic segmentation layout from scratch, then synthesizes a realistic scene conditioned on that layout. For the former, we use an unconditional progressive segmentation generation network that captures the distribution of realistic semantic scene layouts. For the latter, we use a conditional segmentation-to-image synthesis network that captures the distribution of photo-realistic images conditioned on the semantic layout. When trained end-to-end, the resulting model outperforms state-of-the-art generative models in unsupervised image synthesis on two challenging domains in terms of the Frechet Inception Distance and ´ user-study evaluations. Moreover, we demonstrate the generated segmentation maps can be used as additional training data to strongly improve recent segmentation-to-image synthesis networks.
% ●	Our Semantic Bottleneck GAN first unconditionally generates a pixel-wise semantic label map of a scene (i.e. for each spatial location it outputs a class label), and then generates a realistic scene image by conditioning on that semantic map. By factorizing the task into these two steps, we are able to separately tackle the problems of producing convincing segmentation layouts (i.e. a useful global structure) and filling these layouts with convincing appearances (i.e. local structure). When trained end-to-end, the model yields samples which have a coherent global structure as well as fine local details. 
% ●	GANs for discrete domains have been investigated in several works [22, 43, 24, 6, 26].
% ●	we propose an alternative approach that constructs semantic layout as an intermediate representation between text and image. Semantic layout defines a structure of scene based on object instances and provides fine-grained information of the scene, such as the number of objects, object category, location, size, shape, etc. (Figure 1). By introducing a mechanism that explicitly aligns the semantic structure of an image to text, the proposed method can generate complicated images that match complex text descriptions. In addition, conditioning the image generation on semantic structure al

% ●	lows our model to generate semantically more meaningful images that are easy to recognize and interpret. Our model for hierarchical text-to-image synthesis consists of two parts: the layout generator that constructs a semantic label map from a text description, and the image generator that converts the estimated layout to an image using the text.

% ●	The generated layout is then used to guide the image generator for pixel-level synthesis. The box generator, shape generator and image generator are implemented by independent neural networks, and trained in parallel with corresponding supervisions. First, the semantic layout provides instancewise annotations on generated images, which can be directly exploited for automated scene parsing and object retrieval. Second, 
% ●	
% ●	it is important that the structure of the generative model closely resembles the underlying generative process. Deep generative models seek to recover the process with which the observed data was generated. In this work, we investigate object compositionality for Generative Adversarial Networks (GANs) (Goodfellow et al., 2014) 1 . We investigate a minimal modification to a standard neural network generator that incorporates the right inductive bias and find that it reliably learns to generate images as compositions of objects.

% Such local attention is key to limiting the memory and computation consumed by the model, facilitating successful application of self-attention throughout the network, including early high-resolution layers. Our work builds on these results and explores a broader variety of self-attention formulations. 

% Learning good representations of complex visual scenes is a challenging problem for artificial intelligence that is far from solved. Recent breakthroughs in unsupervised representation learning (Higgins et al., 2017a; Makhzani et al., 2015; Chen et al., 2016) tend to focus on data where a single object of interest is placed in front of some background (e.g. dSprites, 3D Chairs, CelebA). 

% We consider semantic image synthesis, which aims at generating photorealistic images conditioned on semantic layouts. It has wide applications on controllable image synthesis and interactive image manipulation. State-of-the-art methods are mostly based on Generative Adversarial Networks (GAN)

% We believe that one fruitful approach to improve generalization in machine learning is to learn compositional representations in an unsupervised manner.

% Our generator starts from a learned constant input and adjusts the “style” of the image at each convolution layer based on the latent code, therefore directly controlling the strength of image features at different scales

% ****** To gain better control over the synthesis process, many works investigate how factors of variation can be disentangled without explicit supervision. They either modify the training objective [9, 39, 70] or network architecture [38], or investigate latent spaces of well-engineered and pre-trained generative models [1, 16, 23, 26, 33, 77, 95]. All of these works, however, do not explicitly model the compositional nature of scenes.

% GAN-based Image Synthesis: Generative Adversarial Networks (GANs) [24] have been shown to allow for photorealistic image synthesis at resolutions

% we advocate to model the formation process directly in 3D for better disentanglement and more controllable synthesis.


% Most approaches, however, do not consider the compositional nature of scenes and operate This often leads to entangled representations 

% he ability to generate and manipulate photorealistic image content is a long-standing goal of computer vision and graphics.

% most existing approaches do not specifically model objects and their relations in images and thus have difficulties in generating complex scenes such as those in the COCO dataset


% Deep generative models (DGMs) (Kingma & Welling, 2013; Goodfellow et al., 2014; Li et al., 2015) have made a great progress in image generation.  By incorporating valid structures explicitly, images with complicated relations can be generated conditionally on these complicated structures. Besides, with these highly-interpretable structures, a better understanding of scene generation can be got, and a set of operations, such as moving objects, changing locations, become possible. Indeed, Mirza & Osindero (2014) and Li et al. (2017) introduce conditional variables to generative models as an input, and synthesize images conditionally. But using a one-hot conditional variable is far from modeling the relations within a complicated realistic image.

% Current generative frameworks use end-to-end learning and generate images by sampling from uniform noise distribution. However, these approaches ignore the most basic principle of image formation: images are product of: (a) Structure: the underlying 3D model; (b) Style: the texture mapped onto structure. In this paper, we factorize the image generation process and propose Style and Structure Generative Adversarial Network (S2 -GAN). Our S2 -GAN has two components: the StructureGAN generates a surface normal map; the Style-GAN takes the surface normal map as input and generates the 2D image.

% Modern Generative Adversarial Networks (GANs) are able to produce a wide variety of highly realistic synthetic images. The phenomenal success of these generative models underscores the need for a better understanding of what kinds of control these models offer over the generated data. 


% ●	Sketching as Discovery https://www.jstor.org/stable/pdf/10.5406/jaesteduc.46.1.0001.pdf?casa_token=XQXgRj3Fc5sAAAAA:XSg84ch5P6LSFTgytXXsoZK48-OouJqyrtwD1EmNj8gOdd4DsD4xefETkzR26_-sLNu8FHj94t50Ggaa9a3qviohmBz2H3Wieiv7RKrRwnty6s0Jktg 

% ●	Like a painter that first draws a rough sketch and only then fills in the details. 

% ●	We explore a new problem of controllable sketch-based image editing, to adapt edge-based models to human-drawn sketches, where the users have the freedom to balance the sketch faithfulness with the output verisimilitude. We propose a sketch refinement method using coarse-to-fine dilations, following the drawing process of artists in real world. We propose a style-based network architecture, which successfully learns to refine the input sketches into diverse and continuous levels.

% ●	Humans have a remarkable ability to “see the infinite world with finite means” [26, 2]. From perceiving a limited set of low-level visual primitives, they can productively compose unlimited higher-level visual concepts, from which an understanding of a viewed scene can be formed.
% ●	sketch refinement method. Modelling the rough sketch as a drawable region via


% ●	Reevaluate memory planning aids, think of how a kid draw a picture of a person as a stick figure reflecting its conceptual understanding of the the object  or of a simple scene with a sun and a house  children's early conceptions of the human body, to be enriched by
% ●	the addition of other body parts. Taking inspiration and allowing into the thought process but at the same time still being computationally efficient, disentangleed
% ●	Sketching is a tool that supports the tacit, complex cognitive processes involved in sense-making, creative discovery, and problem solving.
% ●	Drawing sketches while designing plays an essential role in crystallising design ideas. Past literature has revealed important aspects of sketching that facilitate design processes. There has been no empirical study, however, to reveal how sketches are involved in the very process in which the structures of designers’ actions are dynamically formed. 

% We have devised a general scheme to code designers’ actions belonging to different cognitive levels. Based on the scheme, we analyzed the process of a practicing architect. We found evidence that suggests the following insights. First, the role of sketching is mostly to leave ideas on paper for later inspection and thus perception, rather than to give simultaneous incentives for perception. Second, the role of perception is to stimulate functional thoughts, especially in the phase of detailed exploration. Third, therefore, design behaviors are situated in the physical setting in which designers draw and perceive. Based on these insights, we have proposed the concept of a set of different types of design support tools. They should assist designers’ actions to draw and perceive while maintaining the situatedness of design behaviors.

% ●	Quick, gestural drawing—that is, sketching—unlike these other symbol systems, is also continuous. It emphasizes configural rather than featural information. As neuroscientist Vinod Goel explains, sketching is replete and dense. Its indeterminacies and gaps reflect the way we actually think through problems and provide openings for the new and unforeseen.36  Ambiguity is not only tolerated but cultivated by expert practicioners in order to make room for the draftsman to be surprised by her own work. Cognitive scientists have studied the drawing practices of experts who use rough sketches to inspire new design solutions. More than a mere aid to short-term memory, sketches are not just about lightening cognitive load, or even making new combinations. Sketches support radical restructuring of percepts and concepts, stimulating new analogies and leading the way to innovation and invention. Through disassemb Suwa and Tversky define “constructive perception” as a metacognitive skill that can be honed through practice. Experts can generate new interpretations of ambiguous figures, reorganizing parts to form new wholes, and find new meanings through alternative associations or frames of reference. Openness and fluency of analogical thought seems to be gained through experience.39 

% ●	The emergence of sophisticated digital systems that support the generation of complex graphical models has changed how people use freehand sketching as a tool in designing and problem solving. While digital technologies offer exciting alternatives for expressing design ideas and communicating visually, the ability to create visual images using freehand interactions remains a fundamental skill that has central importance in design and technology classrooms. The value in a sketch is much more than the generated visual image. Sketching is a tool that supports the tacit, complex cognitive processes involved in sense-making, creative discovery, and problem solving.
% Through an analysis of contemporary literature, this chapter examines the nature of sketching through both visual cognition and skills building lenses. Firstly, a foundation is outlined in relation to the nature of visual mental images and how these are generated and externalized during drawing and sketching. Secondly, drawing and sketching are defined and the pedagogical considerations for developing these skills are described using a theoretical model for developing expertise.



% related:


% ●	Modular GAN. 
% ●	model can learn discrete, self-contained, interchangeable representations of multiple objects in a scene. We also found that the learned latent features of each object representation formed a disentangled code that separated the underlying factors of variation One limitation of this work is that the latent objects are assumed to be independent, which is obviously inconsistent with the tremendous statistical structure among objects in real scenes. Future work will tackle the task of learning not just about objects, but about their relations, interactions, and hierarchies in a unsupervised setting.
% 




% ●	simple scenes recursively, building object after object, and Sbai et al. 2018 [48] decompose an image into single-colored strokes for vector graphics. While iterative processes have the advantage of being able to handle an arbitrary number of objects, they are also more unstable and difficult to train. Most of those can either only be used in generation [56], or only handle very simple objects [4, 14, 18]. As a proof of concept, we decided to first ignore this additional difficulty by only handling a set number of objects but our model can naturally be extended with an iterative composition process. This choice is common among works that, like ours, focus on other aspects of image compositionality. Van Steenkiste et al. 2018 [52] advocates for a generative framework that accounts for relationship between objects. While they do produce masks as part of their generative process, they cannot segment a given image. Closer to our setup, the very recent IODINE [18] propose a VAE adapted for multi-objects representations. Their learned representations include a scene decomposition, but they need a costly iterative refinement process whose performance have only been demonstrated on simulated datasets and not real images. Like ours, some prior work have tried to find segmentation mask by recomposing new images. SEIGAN [42] and Cut & Paste [45] learns to separate object and background by moving the region corresponding to the object to another background and making sure the image is still realistic. These methods however, need to have access to background images without objects, which might not be easy to obtain



% Related work Conditional, transformers and compositonal
% ●	[20, 22, 24, 25, 33, 57, 59, 60], where both input and output are images. Compared to earlier non-parametric methods [7, 16, 23], learning-based methods typically run faster during test time and produce more realistic results. In this work, we focus on . We assume the training dataset contains registered segmentation masks and images. With the proposed spatially-adaptive normalization, our compact network achieves better results compared to leading methods ●	    
% ●	Having more control over the general image layout can lead to a higher quality of images (Reed et al., 2016a; Hong et al., 2018b) and is also an important requirement for semantic image manipulation (Hong et al., 2018a; Wang et al., 2018). Approaches that try to exert some control over the image layout utilize Generative Adversarial Nets (Goodfellow et al., 2014), Refinement Networks (e.g. Chen & Koltun (2017); Xu et al. (2018a)), recurrent attention-based models (e.g. Mansimov et al. (2016)), autoregressive models (e.g. Reed et al. (2016c)), and even memory networks supplying the image generation process with previously extracted image features (Zhang et al., 2018b). ●	
% Besides GANs, Chen & Koltun (2017) proposed to use a cascaded refinement network (CRN) for high-resolution semantic image synthesis, and SIMS (Qi et al., 2018) extended it with a non-parametric component, serving as a memory bank of source material to assist the synthesis. Further, Li et al. (2019) employed implicit maximum likelihood estimation (Li & Malik, 2018) to increase the variety of the CRN model. However, these approaches still underperform in comparison to state-of-the-art GAN models. Therefore, next we focus on the recent GAN architectures for semantic image synthesis.

% ●	Perceptual losses. Gatys et al. (2015); Gatys et al. (2016); Johnson et al. (2016) and Bruna et al. (2016) were pioneers at exploiting perceptual losses to produce high-quality images for superresolution and style transfer using convolutional networks. For semantic image synthesis, the VGGbased perceptual loss was first introduced by CRN, and later adopted by Pix2pixHD. Since then, it has become a default for training the generator (Park et al., 2019; Liu et al., 2019; Tan et al., 2020; Tang et al., 2020a). As the perceptual loss is based on a VGG network pre-trained on ImageNet (Deng et al., 2009), methods relying on it are constrained by the ImageNet domain and the representational power of VGG. With the recent progress on GAN training, e.g. by architecture designs and regularization techniques, the actual necessity of the perceptual loss requires a reassessment. 

	%  and sketches with color [42] 
% ●	Initially, GANs were only capable of generating samples drawn from a random distribution [10], but soon multiple models emerged able to perform conditional image synthesis [29,33]. For all the aforementioned models, the user can control the output image by altering the conditional information. Nonetheless, they are not suitable for manipulating an existing image, as they do not consider an image as an input.

% ●	Generative Adversarial Networks . (GANs) [Goodfellow et al. 2014] learn to automatically synthesize realistic image samples [Karras et al. 2018; Miyato et al. 2018]. GANs have enabled several userguided image synthesis tasks such as generating images from user sketches [Isola et al. 2017; Sangkloy et al. 2017], creating face animation [Geng et al. 2018; Nagano et al. 2018], synthesizing photos from language description [Zhang et al. 2017a], and interactively manipulating objects in a generated scene [Bau et al. 2019; Park et al.
% ●	In Reed et al. (2016a), GAN based image generation is conditioned on text and the region in the image where the text manifests, specified during training via keypoints or bounding boxes. While not the focus of our work, the model proposed in this paper can be easily extended to take into account these forms of supervision.
% ●	Generating semantic layout not only improves quality of text-to-image synthesis, but also provides a number of potential benefits. First, the semantic layout provides instancewise annotations on generated images, which can be directly exploited for automated scene parsing and object retrieval. Second, it offers an interactive interface for controlling image generation process; users can modify the semantic layout to generate a desired image by removing/adding objects, changing size and location of objects, etc.

% ●	Layouts to Image Previous methods commonly rely on intermediate pixel-wise semantic label maps generated via a mask regression (object shape) and a box regression network (object position) trained with an L1 objective [13, 2] or an adversarial loss [11]. The final images are then produced via a series of convolutional “refinement” layers [13, 2] or a pre-trained SPADE [21] model. In contrast, [26, 27, 28] generate scenes in a GAN setting. The generator is conditioned on the scene layout and mask predictors via a layout-aware norm, inspired by StyleGAN [15]. [28] further introduce a differentiable graph-scene matching loss to enhance the separation of objects. Orthogonal to these approaches, we avoid intermediate steps and after compressing high-frequency image details (e.g. textures) into our first stage, we model the data distribution in an abstract latent space, rendering auxiliary steps unnecessary.
% ●	. These methods give stunning results but struggle to faithfully reproduce complex sentences with many objects and relationships. To overcome this limitation we propose a method for generating images from scene graphs,
 
% ●	As a step toward these goals, there has been exciting re-cent progress on text to image synthesis [41, 42, 43, 59] by combining recurrent neural networks and Generative Adversarial Networks [12] to generate images from natural language descriptions. These methods can give stunning results on limited domains, such as fine-grained descriptions of birds or flowers. However as shown in Figure 1, leading methods for generating images from sentences struggle with complex sentences containing many objects. A sentence is a linear structure, with one word following another; however as shown in Figure 1, the information conveyed by a complex sentence can often be more explicitly represented as a scene graph of objects and their relationships. Scene graphs are a powerful structured representation for both images and language; they have been used for semantic image retrieval [22] and for evaluating [1] and improving [31] image captioning; methods have also been developed for converting sentences to scene graphs [47] and for predicting scene graphs from images [32, 36, 57, 58]. In this paper we aim to generate complex images with many objects and relationships by conditioning our generation on scene graphs, allowing our model to reason explicitly about objects and their relationships.

% ●	Recently, generative adversarial networks (GAN) [6] have shown stunning results in generating photorealistic images of faces [16, 17] and simple objects [34, 1, 22]. However, generating photorealistic images for complex scenes with different types of objects and stuff remains a challenging problem. 
%  State-of-the-art methods are mostly based on Generative Adversarial Networks (GAN).


% ●	. In addition, Semantic Bottleneck GAN strongly improves the performance of the state-of-the-art semantic image synthesis model in synthesizing photo-realistic images from ground truth segmentations.

% In this paper, we formulate every object manipulation operator (e.g., add/remove) as an unpaired image-to-image translation and build upon the seminal work of CycleGAN [55].


% ●	Generative Adversarial Networks (GANs) [15] have been widely used for image generation [23, 58, 7, 24, 17, 13, 44, 30, 43]. A vanilla GAN has two important components, i.e., a generator and a discriminator. The goal of the generator is to generate photo-realistic images from a noise vector, while the discriminator is trying to distinguish between the real and the generated image. To synthesize user-specific images, Conditional GAN (CGAN) [32] has been proposed. A CGAN combines a vanilla GAN and an external information, such as class labels [34, 35, 9], text descriptions [27, 59, 26], object keypoint [39, 47], human body/hand skeleton [1, 46, 3, 64], conditional images [63, 21], semantic maps [53, 48, 36, 52], scene graphs [22, 60, 2] and attention maps [58, 31, 45].
%$ ●	 and images [23, 56, 31, 47, 47, 39]. Our work is built on the conditional GANs with image inputs, which aims to tackle image-to-image translation problems

% ●	Conditional GANs [20] generate appealing images in a variety of applications including image to image translation both in the case of paired [10] and unpaired data [38, 39], inpainting missing image regions [22, 32], generating photorealistic images from labels [20, 21], and solving for photo super-resolution [15, 14].

% Similar ideas have been applied to various tasks such as generating photographs from sketches [30] or from attribute and semantic layouts [16].

% ●	Recent methods adopt the same idea for conditional image generation applications, such as text2image [41], image inpainting [38], and future prediction [36], as well as to other domains like videos [54] and 3D data [57]. The key to GANs’ success is the idea of an adversarial loss that forces the generated images to be, in principle, indistinguishable from real photos. This loss is particularly powerful for image generation tasks, as this is exactly the objective that much of computer graphics aims to optimize. We adopt an adversarial loss to learn the mapping such that the translated images cannot be distinguished from images in the target domain.
% ●	Conditional Image Generation. Most of these methods use a multi-stage coarse-to-fine strategy to infer the image appearances of all semantic layouts in the input or intermediate results at the same time

% ●	generators from contradicting each other and alleviates the mode collapse problem of GANs. In this paper, we formulate every object manipulation operator (e.g., add/remove) as an unpaired image-to-image translation and build upon the seminal work of CycleGAN [55]. Our work offers extra elements over the above image-to-image translation approaches by building composable modules that perform different object manipulation operations, generating a layered image representation or predicting the depth ordering of the objects in the image. Image layers. Decomposing an image into layers is a task that was already addressed in the 90s [10, 20, 42, 43, 46]. More recently, Yang et al. [51] proposed a layered model for object detection and segmentation that estimates depth ordering and labeling of the image pixels. In [50], the authors use the concept of image layers and propose a layered GAN model that learns to generate background and foreground images separately and recursively and then compose them into a final composite image. Several approaches have been also proposed for the amodal detection [25] or segmentation [15, 30, 57], the task of detecting or segmenting the full extent of an object including any invisible and occluded parts of it. The recent work of Ehsani et al. [13] tries not only to segment invisible object parts but also to reveal their appearance.


% ●	To generate complicated images, image-to-image translation based on GANs are proposed to generate image conditionally.   Pix2pixHD (Wang et al., 2017) introduces multi-scale discriminators and an instance encoder to pix2pix, so as to generate high resolution realistic images conditioned on instance segmentation maps. Besides that, pix2pixHD enables users to edit image structures by manipulating instance maps.
% ●	Most existing GAN-based image systems focus on synthesis realism in appearance domain [27], [32]. For instance, CycleGAN [3] proposes a cycle-consistent adversarial network for realistic image-to-image translation, and so do other related GANs [4], [33], [34], [35], [36], [37], [38]. LR-GAN [39] synthesizes images by introducing spatial transformer networks (STNs)
% ●	Conditional Generative Adversarial Networks (cGANs) have emerged as a powerful method for generating images conditioned on a given input. The input cue could be in the form of an image [10, 38, 17, 2, 30, 22], a text phrase [34, 25, 24, 12] or a class label layout [20, 21, 1]. The goal in most of these GAN instantiations is to learn a mapping that translates a given sample from the source distribution to generate a sample from the output distribution. This primarily involves transforming either a single object of interest (apples to oranges, horses to zebras, label to image, etc.) or changing the style and texture of the input image (day to night, etc.). However, these direct transformations do not capture the fact that a natural image is a 2D projection of a composition of multiple objects interacting in a 3D visual world. Here, we explore the role of compositionality in GAN
% ●	Despite significant recent progress on generative models, controlled generation of images depicting multiple and complex object layouts is still a difficult problem. Among the core challenges are the diversity of appearance a given object may possess and, as a result, exponential set of images consistent with a specified layout. To address these challenges, we propose a novel approach for layout-based image generation; we call it Layout2Im.
% ●	Image generation of complex realistic scenes with multiple objects and desired layouts is one of the core frontiers for computer vision. Existence of such algorithms would not only inform our designs for inference mechanisms, needed for visual understanding, but also provide practical application benefits in terms of automatic image generation for artists and users.


% ●	For these reasons, image generation algorithms have been a major focus of recent research. Of specific relevance are approaches for text-to-image [11, 15, 25, 33, 41, 47] generation. By allowing users to describe visual concepts in natural language, text-to-image generation provides natural and flexible interface for conditioned image generation. However, existing text-to-image approaches exhibit two drawbacks: (i) most approaches can only generate plausible results on simple datasets such as cats [49], birds [44] or flowers [30]. Generating complex, real-world images such as those in COCO-Stuff [1] and Visual Genome [19] datasets remains a challenge; (ii) the ambiguity of textual description makes it more difficult to constrain complex generation process, e.g., locations and sizes of different objects are usually not given in the description. Scene graphs are powerful structured representations that encode objects, their attributes and relationships. In [14] an approach for generating complex images with many objects and relationships is proposed by conditioning the generation on scene graphs. It addresses some of the aforementioned challenges. However, scene graphs are difficult to construct for a layman user and lack specification of core spatial properties, e.g., object size / position. To overcome these limitations, we propose to generate complicated real-world images from layouts, as illustrated in Figure 1. By simply specifying the coarse layout
% ●	Conditional Image Generation. Conditional image generation approaches generate images conditioned on additional input information, including entire source image [13, 23, 32, 46, 50, 51, 52], sketches [13, 36, 43, 45, 52], scene graphs [14], dialogues [16, 37] and text descriptions [25, 33, 41, 47]. Variational Autoencoders (VAEs) [18, 25, 40], autoregressive models [31, 42] and GANs [13, 27, 43, 51] are powerful tools for conditional image generation and have shown promising results. However, many previous generative models [13, 32, 36, 45, 46, 51] tend to largely ignore the random noise vector when conditioning on the same relevant context, making the generated images very similar to each other.

% ●	Image Generation from Layout. The use of layout in image generation is a relative novel task. and the output images, or as a complementary feature for image generation based on context (e.g., text [15, 34, 41], shape and lighting [6]). 

% ●	Recent conditional generators feed the class identifier through a separate embedding network to a large number of layers in the generator [46], while the latent is still provided though the input layer. A few authors have considered feeding parts of the latent code to multiple generator layers [9, 5]. In parallel work, Chen et al. [6] “self modulate” the generator using AdaINs, similarly to our work, but do not consider an intermediate latent space or noise inputs.
% ●	(flow) Conditional GANs. A signi€cant invention for image manipulations are conditional GANs (CGANs). To add conditional information as input, CGANs (Mirza and Osindero 2014) learn a mapping G : x, z → y from an observed input x and a randomly sampled vector z to an output image y. . Other notable works (Nie et al. 2020; Siarohin et al. 2020; Zakharov et al. 2019) produce high quality image animations and manipulations. CGANs can be trained even with unpaired training data using cycle-consistency loss (Kim et al. 2017; Yi et al. 2017; Zhu et al. 2017a). Œey can be used as a building block for image editing, for example, by using a generator G to translate a line drawing or semantic label map to a realistic-looking output image. CGANs have given rise to many application speci€c modi€cations and re€nements
% ●	Image-to-image translation. Image-to-image translation networks have been proposed to translate an image from a source domain into a target domain. Isola et al. [11] designed a general image-to-image translation framework named pix2pix [11] to map semantic label maps or edge maps into photos. Follow-ups involve the diversification of the generated images [39], high-resolution translation [30], and multi-domain translation [4]. This framework requires that images in two domains exist as pairs for training. Zhu et al. [38] suggested a cycle consistency constraint to map the translated image back to its original version, which successfully trained CycleGAN on unpaired data. By assuming a shared latent space across two domains, UNIT [16] and MUNIT [10] are proposed upon CycleGAN to improve the translation quality and diversity.
% ●	(sp2p)  Since then, their work has been extended for many scenarios: high-resolution synthesis [42], unsupervised learning [31, 50, 24, 29], multi-modal image synthesis [7, 15, 51], multi-domain image synthesis [6, 7], and conditional image synthesis [35, 53, 32, 5, 26].


% ●	 The approach thus functions as a rendering engine that takes a two-dimensional semantic specification of the scene and produces a corresponding photographic image
% ●	Conditional Image Generation. Various approaches have been proposed to control the generation process by conditioning on a class label (Odena, Olah, and Shlens 2017), an attribute vector (Kaneko, Hiramatsu, and Kashino 2017; Ding, Sricharan, and Chellappa 2018), a text description (Reed et al. 2016a; Johnson, Gupta, and Fei-Fei 2018), or a semantic map (Isola et al. 2017; Hong et al. 2018). 
% Reed et al. learn to control the foreground object location by conditioning on bounding boxes and keypoint coordinates. Isola et al. propose conditional adversarial networks as a general purpose solution to image-to-image translation problems. Their model can generate a scene from a semantic layout map similar to our work. Nevertheless, the image diversity and the limited control over scene elements are limited. Wang et al. address these limitations of previous conditional models and propose a feature-embedding approach using additional encoder network in order to improve the diversity and controllability. Similar to our method, their method allows an element-level control; however, they use pre-defined low-dimensional feature map to control the appearance of the elements which may limit the diversity. Park, Yoo, and Kwak introduce a new method to learn to generate a foreground object image by conditioning on both the text description, the foreground object mask, and the given background image without altering it. This is the most relevant work to our paper. However, the method can only generate a single foreground object when the background image is given. In contrast, our framework can generate both a background and an arbitrary number of foreground objects. 
% ●	Wang and Gupta [47] synthesize 128×128 images of indoor scenes by factorizing the image generation process into synthesis of a normal map and subsequent synthesis of a corresponding color image.
% ●	In this work, we model a distribution of potential results, as many of these problems may be multimodal in nature. We start with the pix2pix framework [20], which has previously been shown to produce highquality results for various image-to-image translation tasks However, the quality has been attained at the expense of multimodality, as the generator learns to largely ignore the random noise vector when conditioned on a relevant context [20, 34, 40, 45, 47, 55]. In fact, it has even been shown that ignoring the noise leads to more stable training [20, 29, 34].


% ●	Generative Image Models fall into three recent categories: Generative Adversarial Networks (GANs) [12, 40] jointly learn a generator for synthesizing images and a discriminator classifying images as real or fake; Conditional Image Synthesis conditions generation on additional input. GANs can be conditioned on category labels by providing labels as an additional input to both generator and discriminator [10, 35] Reed et al. [42] generate images from text using a GAN; Zhang et al. [59] extend this approach to higher resolutions using multistage generation. Related to our approach, Reed et al. generate images conditioned on sentences and keypoints using both GANs [41] and multiscale autoregressive models [43]; in addition to generating images they also predict locations of unobserved keypoints using a separate generator and discriminator operating on keypoint locations. Chen and Koltun [6] generate high-resolution images of street scenes from ground-truth semantic segmentation using a cascaded refinement network (CRN) trained with a perceptual feature reconstruction loss [9, 21]; we use their CRN architecture to generate images from scene layouts. Related to our layout prediction, Chang et al. have investigated text to 3D scene generation [4, 5]; other approaches to image synthesis include stochastic grammars [20], probabalistic programming [27], inverse graphics [28], neural de-rendering [55], and generative ConvNets [56].  Compared to leading methods which generate images from text descriptions, generating images from structured scene graphs rather than unstructured text allows our method to reason explicitly about objects and relationships, and generate complex images with many recognizable objects.
% ●	Sentence-conditioned image generation. A variety of models have proposed to generate an image given a sentence. Reed et al. [25] use a GAN [7] that is conditioned on a text encoding for generating images. Zhang et al. [30] propose a GAN based image generation framework where the image is progressively generated in two stages at increasing resolutions. Reed et al. [24] perform image generation with sentence input along with additional information in the form of keypoints or bounding boxes. 
% ●	While scene layout generation in this work predicts probability distributions for bounding box layout, it fails to model the stochasticity intrinsic in predicting each bounding box. Gupta et al. [8] use an approach similar to [11] to predict layouts for generating videos from scripts. Johnson et al. [12] uses the scene graph generated from the input sentence as input to the image generation model. Given a scene graph, their model can generate only one scene layout. Deng et al. [6] propose PNP-Net, a VAE framework to generate image of an abstract scene from a text based program that fully describes it. While PNP-Net is a stochastic model for generation, it was tested on synthetic datasets with only a small number of classes. Furthermore, it tries to encode the entire image into a single latent code whereas, in LayoutVAE, we break down just the layout generation step into two stages with multiple steps in each stage. Based on these reasons, it is unclear whether PNP-Net can scale up to real world image datasets with a large number of classes. Tao et al. [29] propose a GAN based model with attention for sentence to image generation. The more recent work from Li et al. [19] follow a multi-stage approach similar to [11] to generate an image from a sentence, with the key novelty of using attention mechanisms to create more realistic objects in the image. Layout generation in other contexts. Chang et al. [3] propose a method for 3D indoor scene generation based on text description by placing objects from a 3D object library, and is later improved in [2] by learning the grounding of more detailed text descriptions with 3D objects. Wang et al. [28] use a convolutional network that iteratively generates a 3D room scene by adding one object at a time. Qi et al. [23] propose a spatial And-Or graph to represent indoor scenes, from which new scenes can be sampled. Different from most other works, they use human affordances and activity information with respect to objects in the scene to model probable spatial layouts. Li et al. [18] propose a VAE based framework that encodes object and layout information of indoor 3D scenes in a latent code. During generation, the latent code is recursively decoded to obtain details of individual objects and their layout. More recently, Li et al. [17] proposed LayoutGAN, a GAN based model that generates layouts of graphic elements (rectangles, triangles etc.). While this work is close to ours in terms of the problem focus, LayoutGAN generates label sets based on input noise, and it cannot generate layout for a given set of labels. Placing objects in scenes. Lee et al. [16] propose a conditional GAN model for the problem of adding the segmentation mask of a new object to the semantic segmentation of an image. Lin et al. [20] address a similar problem of adding an RGB mask of an object into a background image.
% ●	Previous approaches with conditional generative adversarial networks (GAN) show state-of-the-art performance on this task, which  W
% ●	enhance the spatial semantic alignment between the generated images and the input semantic layout.




% ●	strong style and layout controllability.  showing insights of how the proposed model generates complex scenes in high quality. Compared with the previous work, our object-driven attention is more robust and interpretable, and significantly improves the object generation quality in complex scenes.
% ●	To explicitly encode the semantic layout into the generator, [9] proposes to decompose the generation process into two steps, in which it first constructs a semantic layout (bounding boxes and object shapes) from the text and then synthesizes an image conditioned on the layout and text description. [12] also proposes such a two-step process to generate images from scene graphs, and their process can be trained end-to-end
% ●	To explicitly encode the semantic layout into the generator, [9] proposes to decompose the generation process into two steps, in which it first constructs a semantic layout (bounding boxes and object shapes) from the text and then synthesizes an image conditioned on the layout and text description. [12] also proposes such a two-step process to generate images from scene graphs, and their process can be trained end-to-end
% ●	In this work, we employ scene graphs with per-object location and appearance attributes as an accessible and easyto-manipulate way for users to express their intentions, see Fig. 1. The what aspect is captured hierarchically: objects are defined as belonging to a certain class (horse, tree, boat, etc.) and as having certain appearance attributes. These attributes can be (i) selected from a predefined set obtained by clustering previously seen attributes, or (ii) copied from a sample image. The where aspect, is captured by what is often called a scene graph, i.e., a graph where the scene objects are denoted as nodes, and their relative position, such as “above” or “left of”, are represented as edge types.
% ●	we allow for much more control and freedom to the object selection mechanism, (
% ●	this effect is amplified by the ability of the users to manipulate the resulting image

% ●	Image generation techniques based on GANs [3] are constantly improving in resolution, visual quality, the diversity of generated images, and the ability to cover the entire visual domain presented during training. In this work, we address conditional image generation, i.e., the creation of images that match a specific input. Earlier work in conditional image generation includes class based image generation [16], which generates an image that matches a given textual description [18, 26]. In many cases, the conditioning signal is a source image, in which case the problem is often referred to as image translation. Pix2pix [7] is a fully supervised method that requires pairs of matching samples from the two domains. The Pix2pixHD architecture that was recently presented by [25] is highly influential and many recent video or image mapping works employ elements of it, including our work.

% ●	Also related is the synthesis of images from a given input layout of bounding boxes (and not one that is inferred by a network from a scene graph), which was very recently studied by [28] for small 64x64 images. In another line of work,
% ●	Recently, an interactive tool was introduced based on the novel notion of GAN dissection [1]. This tool allows for the manipulation of well-localized neurons that control the occurrence of specific objects across the image using a drawing interface. By either adding or reducing the activations of these neurons, objects can be added, expanded, reduced or removed. The manipulation that we offer here is both more semantic (less related to specific locations and more to spatial relations between the objects), and more precise, in the sense that we provide full control over the exact instance of the object and not just of the desired class.
% ●	requires multiple reasonings on various visual concepts, such as object category (people and elephants), spatial configurations of objects (riding), scene context (walking through a river), etc., which is much more complicated than generating a single, large object as in simpler datasets [33, 17].

% ●	(Inferring Semantic Layout for Hierarchical Text-to-Image Synthesis)k (GAN) [7] have shown promising results in text-toimage synthesis [21, 23, 34, 6, 4].

% ●	The problem of generating images from pixel-wise semantic labels has been explored recently [3, 10, 12, 22]. In these approaches, the task of image generation is formulated as translating semantic labels to pixels. Isola et al. [10] proposed a pixel-to-pixel translation network that converts dense pixel-wise labels to an image, and Chen et al. [3] proposed a cascaded refinement network that generates high-resolution output from dense semantic labels. Karacan et al. [12] employed both dense layout and attribute vectors for image generation using conditional GAN. Notably, Reed et al. [22] utilized sparse label maps like our metho
% ●	Karacan et al. (2016), Johnson et al. (2018), and Wang et al. (2018) use a scene layout to generate images in which given objects are drawn within their specified segments based on the generated scene layout. This is further extended by Hong et al. (2018a) by making it possible to manipulate images on a semantic level. While these approaches offer a more detailed control over the image layout they heavily rely on a semantic scene layout for the image generating process, often implying complex preprocessing steps in which the scene layout is constructed
% ●	StackGAN: Text to Photo-realistic Image Synthesis with Stacked Generative Adversarial Networks - sketches idea
% ●	Object discovery Our object discovery architecture is closely related to a line of recent work on compositional generative scene models [16, 17, 24–27, 38–44]
% ●	While prior work focuses on a single object, we aim to obtain a holistic scene understanding.
% ●	Some control over the generated results may be obtained via conditioning [21], which requires training the model with annotated data. In contrast, style-based design enables discovering a variety of interpretable generator controls after training the generator. However, current methods require either a pretrained classifier [10, 30, 31, 35], a large set of paired examples [15], or manual examination of many candidate control directions [12], which limits the versatility of these approaches. Furthermore, the individual controls discovered by these methods are typically entangled, affecting multiple attributes, and are often non-local. In this work, our goal is to understand to what degree disentanglement is inherent in style-based generator architectures. Perhaps an even more important question is to how to find these disentangled controls? In particular, can this be done in an unsupervised manner, or with only a small amount of supervision? In this paper we report several findings with respect to these questions.
% ●	Semantic-guided scene generation is a hot research topic covering several main-stream research directions, including cross-view image translation [21, 57, 40, 41, 48, 42] and semantic image synthesis [53, 8, 38, 36].
% ●	image from a semantic map [53, 8, 38, 36], as shown in Fig. 1(top). Recently, Park et al. 
% ●	Stochastic decoder-based models, such as conditional GANs, were recently proposed to alleviate some of these issues. In particular, both Pix2PixHD [39] and SPADE [32] are able to synthesize high-quality scenes using a strong conditioning mechanism based on semantic segmentation labels during the scene generation process. Global structure encoded in the segmentation layout of the scene is what allows these models to focus primarily on generating convincing local content consistent with that structure. 

% ●	In conditional image synthesis one aims to generate images by conditioning on an input which can be provided in the form of an image [18, 47, 3, 5, 25], a text phrase [37, 45, 35, 2, 17], a scene graph [20, 2], a class label or a semantic layout [31, 8, 39, 32]. These conditional GAN methods learn a mapping that translates samples from the source distribution into samples from the target domain.  Our work shares the same high-level idea of decomposing the image generation problem into the semantic layout synthesis and the conditional semantic-layout-to-image synthesis. A key difference is that we focus on unconditional image generation which results in a novel semantic layout generation pipeline and end-to-end network design.
% ●	Image-to-image translation Many researchers have leveraged adversarial learning for image-to-image translation [21], whose goal is to translate an input image from one domain to another domain given input-output image pairs as training data. Compared to L1 loss, which often leads to blurry images [21, 22], the adversarial loss [16] has become a popular choice for many image-to-image tasks [10, 24, 25, 31, 40, 45, 53, 58, 64]. The reason is that the discriminator can learn a trainable loss function and automatically adapt to the differences between the generated and real images in the target domain. For example, the recent pix2pix framework [21] used image-conditional GANs [38] for different applications, such as transforming Google maps to satellite views and generating cats from user sketches. Various methods have also been proposed to learn an image-to-image translation in the absence of training pairs [2, 33, 34, 46, 49, 51, 54, 63]. Recently, Chen and Koltun [5] suggest that it might be hard for conditional GANs to generate high-resolution images due to the training instability and optimization issues. To avoid this difficulty, they use a direct regression objective based on a perceptual loss [11, 13, 22] and produce the first model that can synthesize 2048 × 1024 images. The generated results are high-resolution but often lack fine details and realistic textures. Our method is motivated by their success. We show that using our new objective function as well as novel multi-scale generators and discriminators, we not only largely stabilize the training of conditional GANs on high-resolution images, but also achieve significantly better results compared to Chen and Koltun [5]. Side-by-side comparisons clearly show our advantage (Figs. 1, 7, 8, 9).



% ●	Instead of generation from a random noise, conditional image synthesis refers to the task of generating photo-realistic images conditioned on the input such as texts [18], [19], [20], [21] and images [1], [4], [22], [23], [24], [25]. Our work focuses on a special form of . For this task, many impressive works have been proposed in the past several years. One of the most representative works is pix2pix [4], which proposes a unified image-to-image translation framework based on the conditional generative adversarial network. To further improve its quality or enable more functionality, many following works have appeared, such as pix2pixHD [5], SIMS [26], and SPADE [1]. S Many recent works for different downstream tasks have used this architecture, such as semantic image synthesis [27], [28], [29], portrait synthesis or editing [30], [31] and semantic view synthesis [32]. Other works [33], [34], [35], although not using SPADE directly, are inspired by it to introduce spatial-adaptiveness or approximate spatialadaptiveness into normalization layers. Despite the success of SPADE, its efficiency is often neglected and understudied in the community. In this paper, we conduct an in-depth analysis of its superiority and propose a new efficient and effective normalization layer.
% ●	

% ●	 For example, it is easily possible that the segmentation mask of the desired output image contains a labeled region that is not present in the segmentation mask of the input style image. In this case, the style of the missing region is undefined, which yields low quality results. Further, SPADE  Our first main idea is therefore to control the style of each region individually, i.e., our proposed architecture accepts one style image per region (or per region instance) as input. 

% ●	Image-to-Image Translation. Image-to-image translation is an umbrella concept that can be used to describe many problems in computer vision and computer graphics. As a milestone, Isola et al. [23] first showed that imageconditional GANs can be used as a general solution to various image-to-image translation problems. Since then, their method is extended by several following works to scenarios including: unsupervised learning [56, 31], few-shot learning [32], high resolution image synthesis [47], multimodal image synthesis [57, 22] and multi-domain image synthesis [9]. [29, 5, 16, 39]. To date, the SPADE [39] model (also called GauGAN) generates the highest quality results. In this paper, we will improve SPADE by introducing per-region style encoding.
% ●	Image-to-image translation aims to learn the mapping between two image domains [1,20,22,27,56,57]. These techniques demonstrate a wide range of applications such as image inpainting, image super-resolution, domain adaptation [4,18], and semantic image synthesis [46,35]. In particular, semantic image synthesis learns to generate photo-realistic images conditioned on semantic label maps. the semantic image synthesis frameworks, we aim to synthesize 3D representation of a scene from a single-view semantic segmentation layout.

% ●	Conditional image generation Another relevant line of work is conditional image generation, in particular works using segmentation maps. Pix2pix [14] has shown that image to image translation can give very realistic results in going from a segmentation mask to a real image. Recent improvements, such as CRN [5] and pix2pixHD [23] have shown extensions to higher resolutions. [20] have also shown very convincing translations from segmentation maps to images using a semi-parametric approach. Improvements have also been shown by making use of spatial normalisation in SPADE [19]

% Related work: Layers iterative
% ●	BlockGAN is of particular interest because, via its relatively strong architectural biases, it  . This approximation is  or for scenes such as stacking wooden blocks or cars following a path, where the (object) correlation is strong.
% ●	Sequential Image Generation. A coarse-to-fine generation process can be cast as a sequential image generation process. Denton et al. introduce a sequential model with a  Song, Zhang, and Qi generate a face image from a small face patch iteratively. They refine the image by transformations between two image manifolds. 
% ●	Similar to our method, Lin et al. and Yang et al. adopt a layered structure modeling and compose a scene sequentially. However, Lin et al. focus on finding the appropriate geometric transformation of an object in a background layout, in an iterative manner. In our work, the user defines the geometry of the object and no transformation is involved. Their objective is then orthogonal to ours. Yang et al. focus on the unsupervised discovery of object masks, in a layerwise process. Contrary to our work, the foreground generator produces a foreground mask instead of being conditioned on it. Such a scheme does not provide the same level of controllability and flexibility as ours. Moreover, their experiments were restricted to one object instance per image compared to 2.61 instances per image on average in our case.
% ●	Interpretable image representation. Our work is inspired by prior work on obtaining interpretable visual representations with neural networks [Kulkarni et al., 2015, Chen et al., 2016]. To achieve this goal, DC-IGN [Kulkarni et al., 2015] freezes a subset of latent codes while feeding images that move along a specific direction on the image manifold. A recurrent model [Yang et al., 2015] learns to alter disentangled latent factors for view synthesis. InfoGAN [Chen et al., 2016] proposes to disentangle an image into independent factors without supervised data. Another line of approaches are built on intrinsic image decomposition [Barrow and Tenenbaum, 1978] and have shown promising results on faces [Shu et al., 2017] and objects [Janner et al., 2017]. While prior work focuses on a single object, we aim to obtain a holistic scene understanding.
% ●	Sequential models have been pivotal for improved image generation using variational autoencoders: DRAW (Gregor et al., 2015) uses attention based recurrence conditioning on the canvas drawn so far. In Eslami et al. (2016), a recurrent generative model that draws one object at a time to the canvas was used as the decoder in VAE. These methods are yet to show scalability to natural images. Early compelling results using GANs used sequential coarse-to-fine multiscale generation and classconditioning (Denton et al., 2015). Since then, improved training schemes 
% ●	Our work instead follows a more recent trend by inferring scene decomposition directly from data. Stemming from DRAW [19], many of those approaches [4, 14] use an attention network to read a region of an image and a Variational Auto-encoder (VAE) to partially reconstruct the image in an iterative process in order to flesh out a meaningful decomposition. LR-GAN [56] is able to generate
% ●	Object-aware image synthesis. Recent methods decompose image synthesis into generating components like layers or image patches, and combining them into the final image [31, 53, 56]. This includes conditional GANs that use segmentation masks [43, 52], scene graphs [24], object labels, key points or bounding boxes [20, 45], which have shown impressive results for natural image datasets. Recently, unsupervised methods [3, 14, 15, 29, 53, 58] learned object disentanglement for multi-object scenes on  (single-colour objects, simple lighting, and material). Other approaches successfully separate foreground from background objects in natural images, but make strong assumptions about the size of objects [56] or independent object appearance [4, 8]. These methods treat object components as image patches or 2D layers with corresponding masks, which are combined via alpha compositing at the pixel level to generate the final stage. The work closest to ours learns to generate multiple 3D primitives (cuboids, spheres and point clouds), renders them into separate 2D layers with a handcrafted differentiable renderer, and alpha-composes them based on their depth ordering to create the final image [32]. Despite the explicit 3D geometry, this method does not handle cluttered backgrounds and requires extra supervision in the shape of labelled images with and without foreground objects.
% iterative 

% ●	We present LR-GAN: an adversarial image generation model which takes scene structure and context into account. Unlike previous generative adversarial networks (GANs), the proposed 
% ●	Image layers. Decomposing an image into layers is a task that was already addressed in the 90s [10, 20, 42, 43, 46]. More recently, Yang et al. [51] proposed a layered model for object detection and segmentation that estimates depth ordering and labeling of the image pixels. Several approaches have been also proposed for the amodal detection [25] or segmentation [15, 30, 57], the task of detecting or segmenting the full extent of an object including any invisible and occluded parts of it. The recent work of Ehsani et al. [13] tries not only to segment invisible object parts but also to reveal their appearance.


% ●	In user-guided semantic image editing the user is able to semantically edit an image by adding, manipulating, or removing semantic concepts [3]. Both GANPaint [3] and SinGAN [43] are able to perform such operations: GANPaint [3] by manipulating the neuron activations and SinGAN [43] by learning the internal batch statistics of an image. However, both are trained on a single image and require retraining in order to be applied to another, while our model is able to handle the manipulation of multiple images without retraining. Another simple type of editing is inpainting [13,56,25], where the user masks a region of the image for removal and the network fills it accordingly to the image context. In its classic form the user does not have control over the generated pixel. To address this, other research works guide the generation of the missing areas using edges [55,32] and/or color [37,16] information.
% ●	 early works use hand-designed features, such as Laplacian pyramids for seamless blending (Burt & Adelson, 1983). Hays & Efros (2007) and Isola & Liu (2013) employ nearest-neighbor approaches for scene composition and completion. More recently, a number of deep network architectures have been developed for compositional tasks. For discriminative tasks, Tabernik et al. (2016) and Kortylewski et al. (2020) train CNNs with modified compositional architectures to understand model interpretability and reason about object occlusion in classification. 
% For image synthesis, Mokady et al. (2019) and Press et al. (2020) use an autoencoder to encode, disentangle, and swap properties between two sets of images, while Shocher et al. (2020) mixes images in deep feature space while training the generator. Rather than creating models specifically for image composition or scene completion objectives, we investigate the ability of a . 
% Related to our work, Besserve et al. (2018) estimates the modular structure of GANs by learning a casual model of latent representations, whereas we investigate the GAN’s compositional properties using image inversion. Due to the imprecise nature of image collages, compositing image parts also involves inpainting misaligned regions. However, in contrast to inpainting, in which regions have to be filled in otherwise globally consistent images (Pathak et al., 2016; Iizuka et al., 2017; Yu et al., 2018; Zeng et al., 2020), the composition problem involves correcting inconsistencies as well as filling in missing pixels.
% ●	Image Editing. A recent topic of interest is editing images using generative models. A number of works  (Goetschalckx et al., 2019; Jahanian et al., 2020; Shen et al., 2019; Kingma & Dhariwal, 2018; Karras et al., 2019a; Radford et al., 2015). It is also possible to identify concepts learned in the generator’s intermediate layers by clustering intermediate representations, either using segmentation labels (Bau et al., 2018) or unsupervised clustering (Collins et al., 2020), and change these representations to edit the desired concepts in the output image. Suzuki et al. (2018) use a spatial feature blending approach which mixes properties of target images in the intermediate feature space of a generator. On faces, editing can be achieved using a 3D parametric model to supervise the modification (Tewari et al., 2017; 2020). In our work, we do not require clusters or concepts in intermediate layers to be defined a priori, nor do we need distinct input and output domains for approximate collages and real images, as in image translation tasks (Zhu et al., 2017; Almahairi et al., 2018). Unlike image manipulation using semantic maps (Park et al., 2019; Gu et al., 2019b), our approach respects the style of the manipulation (e.g. the specific color of the sky), which is lost in the semantic map representation. Our method shares commonalities with Richardson et al. (2020), although we focus on investigating compositional properties rather than image-to-image translation. In our approach, we only require a single example of the approximate target property we want to modify and use regression into the latent space as a fast image prior to create a coherent output. This allows us to create edits that are not contingent on labelled concepts, and we do not need to modify or train the generator.
% ●	Scene manipulation and editing. Previous efforts were also made to edit scene images. Laffont et al [18] defined 40 transient attributes and managed to transfer the appearance of a similar scene to the image for editing. Cheng et al [7] proposed verbal guided image parsing to recognize and manipulate the objects in indoor scenes. Karacan et al [15] learned a conditional GAN to synthesize outdoor scenes based on pre-defined layout and attributes. Some other work [19, 43, 13, 20] studied image-to-image translation and can be used to transfer the style of one scene to another. Different from them, we achieve scene manipulation by interpreting the hierarchical semantics emerging from the generative representations of well-trained GANs. Besides image editing, such interpretation also gives us a better insight on how generative models are able to produce photo-realistic synthesis.
% ●	We start by postulating an underlying generative process for images that relies on an assumption of independence between regions of an image we want to detect. This means that replacing one object in the image with another one, e.g. a generated one, should yield a realistic image. We use such a generative model as a backbone for designing an object segmentation model
% ●	can learn interpretable representations on complex datasets where no previous unsupervised approach is known to learn representations of comparable quality.
% ●	Make latent change only to a particular layer
% ●	unsupervised and learns interpretable and disentangled representations on challenging datasets.
% ●	Our findings pave the way to semantically meaningful and well-disentangled image manipulations via simple and intuitive interfaces.

% ●	Generative adversarial networks [18] introduced new possibilities to the field of image generation and synthesis. Currently, state-of-the-art GANs [29, 28, 26, 8] can produce high-resolution synthetic images that are indistinguishable from real images. GANs are also employed in supervised and unsupervised image-to-image translation [24, 45, 35, 49, 9, 34, 23, 10] allowing to transform or edit a given image in various imaginative ways
% ●	(Hierarchy Composition GAN for High-fidelity) In recent years, quite a number of image composition studies have been reported in the field of computer vision, including the synthesis of single objects [8], [9], [10], generation of full-scene images [11], [12], etc. Image composition aims to generate new images by embedding foreground objects into background images. It strives for synthesis realism by adjusting the size and orientation of the foreground objects as well as blending between foreground objects and background images. [13] proposes a model to distinguish natural photographs from automatically generated composite images. [14], [15], [16], [17], [18], [19] investigate the synthesis of scene text images for training better scene text detector and recognizer.
% ●	Image composition is a challenging problem in computer graphics where objects from different images are to be overlaid in one single image. The appearance and geometric differences between these objects are the obstacles that can result in non-realistic composed images

% ●	GANs are utilized for data generation in various domains, including images [27], videos [31], and 3D voxelized data [33]. For images in particular, it has been shown to generate compelling results in a vast variety of conditional image generation problems such as superresolution [16], inpainting [25], image-to-image translation [10, 44, 19], and image editing/manipulation [43]
% ●	Moreover, [12] computed a scene layout from given scene graphs which revealed explicit reasoning about relationships between objects and converted the layout to an output image.
% ●	Image compositing refers to the process of overlaying a masked foreground image on top of a background image. One of the main challenges of image compositing is that the foreground object usually comes from a different scene than the background, and therefore it is not likely to match the background scene in a number of ways that negatively effects the realism of the composite. These can be both appearance differences (due to lighting, white balance, and shading differences) and geometric differences (due to changes in camera viewpoint and object positioning).
% ●	Image inpainting
% ●	Despite the recent success of GANs in synthesizing images conditioned on inputs such as a user sketch, text, or semantic labels, manipulating the highlevel attributes of an existing natural photograph with GANs is challenging for two reasons. First, it is hard for GANs to precisely reproduce an input image. Second, after manipulation, the newly synthesized pixels often do not fit the original image
% ●	Our method can accurately reconstruct the input image and synthesize new content, consistent with the appearance of the input image. 
% imagery 
% render

% ●	We seem to be on the verge of using these generative models for semantic manipulation of natural photographs, which will combine the simplicity of pixel-level editing with flexible semantic manipulations of a scene. The role of deep generative models will be to provide latent semantic representations in which concepts can be directly manipulated and then to preserve image realism when semantic changes are made. This editing scheme will allow users to manipulate a photograph not with physical colors, but with abstract concepts such as object types and visual attributes. For example, a user can add a lit lamp into a bedroom (Figure 1 bottom left) or change the color of a tree’s leaves (Figure 1 bottom right) with a few scribbles.
% ●	Deep visual manipulation Recently, deep neural networks have obtained promising results in various image processing tasks, such as style transfer [13], inpainting [40], colorization [56], and restoration [14]. However, most of these works lack an interface for users to adjust the current result or explore the output space. To address this issue, Zhu et al. [62] developed an optimization method for editing the object appearance based on the priors learned by GANs. Recent works [21, 45, 57] also provide user interfaces for creating novel imagery from low-level cues such as color and sketch. All of the prior works report results on low-resolution images. Our system shares the same spirit as this past work, but we focus on object-level semantic editing, allowing users to interact with the entire scene and manipulate individual objects in the image. As a result, users can quickly create a novel scene with minimal effort. Our interface is inspired by prior data-driven graphics systems [6, 23, 28]. But our system allows more flexible manipulations and produces high-res results in real-time.
% ●	. Several lines of work [Brock et al. 2017; Perarnau et al. 2016; Zhu et al. 2016] propose to manipulate a photo using GANs but only work with a single object (e.g., handbag) at low resolutions (64x64) and often involve post-processing steps. In this work, our method can directly generate a final result and allow semantic manipulations of an entire natural scene
% ●	Deep Image Manipulation. Deep learning has achieved compelling results in many image editing tasks. Recent examples include image inpainting [Iizuka et al. 2017; Pathak et al. 2016; Yu et al. 2018], image colorization [Iizuka et al. 2016; Zhang et al. 2016b], photo stylization [Gatys et al. 2016; Li et al. 2018; Zhu et al. 2017] and photo enhancement [Gharbi et al. 2017; Kim and Park 2018]. Learningbased systems allow real-time computation and require no handcrafted heuristics. Recent work further integrates user interaction into end-to-end learning systems, enabling interactive applications such as user-guided colorization
% ●	This enables new visual effects where training data is not available, such as adding objects and changing the appearance of objects. 
% ●	First, our method requires an optimization be run after each edit,  Second, another challenge is that latent spaces learned by deep neural networks are not fully disentangled, so finding vector operations to express a user intent can remain challenging. Adding or removing an object from a scene may have some interactions with unrelated objects. Some examples of undesirable interaction are illustrated in Figure 11; in these examples, chairs are reduced by zeroing chair-correlated components in the representation, but the rendered results do not cleanly remove all parts of the chairs, and distorted parts that resemble chair legs remain in the result. We also note that our method for varying the appearances of objects can be brittle; certain classes of objects (such as trees) vary more than other classes (such as domes or skies). For example, in Figure (10) we found that dome shape, but not color, could be varied.
% ●	One promising approach for manipulating real images is image-to-image translation (Isola et al., 2017; Zhu et al., 2017; Choi et al., 2018), where the model learns to directly synthesize an output image given a user’s input. However, these methods require pre-defined tasks and heavy supervision (e.g., input-output pairs, class labels) for training, and also limit the user controllability at inference time. Another approach is to utilize pretrained GAN models, by directly optimizing the latent code for an individual image (Abdal et al., 2019; Zhu et al., 2016; Ma et al., 2018; Noguchi & Harada, 2019)
% ●	None of the prior editing can move an object - local edits
% ●	Generative models for content creation The recent progress in generative models has opened interesting avenues for content creation (Brock et al., 2018; Karras et al., 2018), including applications that enable users to fine-tune the generated output (Simon; Zhu et al., 2016; Bau et al., 2018). A by-product the current work is enable users to modify image properties by turning a single knob – the magnitude of the learned transformation in latent space. We further demonstrate that these image manipulations are not just a simple creativity tool; they also provide us with a window into biases and generalization capacity of these models. Applications of latent space editing Image manipulations using generative models suggest several interesting downstream applications.
% ●	High-quality, diverse, and photorealistic images can now be generated by unconditional GANs (e.g., StyleGAN). However, limited options exist to control the generation process using (semantic) aŠributes, while still preserving the quality of the output. Further, due to the entangled nature of the GAN latent space, performing edits along one aŠribute can easily result in unwanted changes along other aŠributes. In this paper, in the context of conditional exploration o
% ●	conditional exploration as an instance of conditional continuous normalizing ƒows in the GAN latent space conditioned by aŠribute features.
% ●	A longstanding goal of Computer Graphics has been to generate high-quality realistic images that can be controlled using userspeci€ed aŠributes. One broad philosophy has been to create detailed 3D models, decorate them with custom materials and texture
% ●	Alternately, in a recent development, generative adversarial networks (GANs) have opened up an entirely di‚erent image generation paradigm. Tremendous interest in this area has resulted in rapid improvements both in speed and accuracy of the generated results. For example, StyleGAN (Karras et al. 2019b), one of the most celebrated GAN frameworks, can produce high resolution images with unmatched photorealism. However, there exist limited options for the user to control the generation process with adjustable aŠribute speci€cations. For example, starting from a real face photograph, how can we edit the image to change the (camera) pose, illumination, or the person’s expression?
% ●	One successful line of research that supports some of the abovementioned edit controls is conditional generation using GANs. In such a workƒow, aŠributes have to be speci€ed directly at (GAN) training time. While the resultant conditional GANs (Choi et al. 2019; Park et al. 2019; Xiao et al. 2018) provide a level of (semantic) aŠribute control, the resultant image qualities can be blurry and fail to reach the quality produced by uncontrolled GANs like StyleGAN. Further, other aŠributes, which were not speci€ed at training time, can change across the generated images, and hence result in loss of (object) identity due to edits.
% ●	Image Editing by Manipulating Latent Codes. A competing approach to conditional GANs is the idea to manipulate latent codes of a pretrained GAN. Radford et al. (2016) observed that interesting
% ●	Image Editing. A recent topic of interest is the ability to edit images using generative models.  (Goetschalckx et al., 2019; Jahanian et al., 2019; Shen et al., 2019; Kingma & Dhariwal, 2018; Karras et al., 2019a; Radford et al., 2015). One may also identify concepts learned in the generator’s intermediate layers by clustering intermediate representations, either using segmentation labels (Bau et al., 2018) or unsupervised clustering (Collins et al., 2020), and change these representations to edit the desired concepts in the output image. Suzuki et al. (2018) use a spatial feature blending approach which mixes properties of target images in the intermediate feature space of a generator. On faces, editing can be achieved using a 3D parametric model to supervise the modification (Tewari et al., 2017; 2020). In our work, we do not require clusters or concepts in intermediate layers to be defined a priori, nor do we need distinct input or output domains as in image translation tasks (Zhu et al., 2017; Almahairi et al., 2018). Furthermore, unlike image manipulation using semantic maps (Park et al., 2019; Gu et al., 2019b), our approach respects the style of the manipulation (e.g. the specific color of the sky), which is lost in the semantic map representation. Our method shares commonalities with Richardson et al. (2020), although we focus on investigating composition rather than image-to-image translation. In our approach, we only require a single example of the approximate target property we want to modify and use regression into the latent space as a fast image prior to create a coherent output. This allows us to create edits that are not contingent on learned concepts, and we do not need to modify or train the generator network.
% ●	Learning an interpretable factorised representation of the independent data generative factors of the world without supervision is an important precursor for the development of artificial intelligence that is able to learn and reason in the same way that humans do
% ●	Latent space manipulations can be seen from several perspectives – how we achieve it, what limits it, and what it enables us to do. Our work addresses these three aspects together, and we briefly refer to each one in related work.  such as smile-vectors and gender-vectors for faces (Radford et al., 2015; Karras et al., 2018).
% ●	An active line of study on GANs interpretability investigates the structure of their latent spaces. Namely, several works (Jahanian et al., 2020; Plumerault et al., 2020; Goetschalckx et al., 2019; Shen et al., 2019) aim to identify semantically meaningful directions, i.e., corresponding to humaninterpretable image transformations. At the moment, prior works have provided enough evidence that a wide range of such directions exists. Some of them induce domainagnostic transformations, like zooming or translation (Jahanian et al., 2020; Plumerault et al., 2020), while others correspond to domain-specific transformations, e.g., adding smile or glasses on face images (Radford et al., 2015).
% ●	Understanding the latent representations of pretrained generators has attracted considerable attention, since it contributes to better GAN architecture design and facilitates controllable manipulation. Bau et al. [5, 3] They further show that in W+ space, early layers control layout, middle layers control the presence of objects, and late layers control final rendering. Collins et al. [7] transfer the appearance of a specific object part from a reference image to a target image, through swapping between style codes. Concurrent work by Xu et al. [34] shows that style space can be used for a variety of discriminative and generative tasks
% ●	Representation learning lies at the core of machine learning research. From the hand-crafted feature engineering prevalent in the past [11] to implicit representation learning of the modern deep learning approaches [23, 14, 38], it is a common theme that the performance of algorithms is critically dependent on the nature of their input representations. Despite the recent successes of the deep learning approaches [14, 38, 13, 30, 31, 29, 28, 19, 37], they are still far from the generality and robustness of biological intelligence [25]. Hence, the implicit representations learnt by these approaches through supervised or reward-based signals appear to overfit to the training task and lack the properties necessary for knowledge transfer and generalisation outside of the training data distribution. Different ways to overcome these shortcomings have been proposed in the past, such as auxiliary tasks [19] and data augmentation [41]. Another less explored but potentially more promising approach might be to use task-agnostic unsupervised learning to learn features that capture properties necessary for good performance on a variety of tasks [4, 26]. In particular, it has been argued that disentangled representations might be helpful [4, 34]. A disentangled representation can be defined as one where single latent units are sensitive to changes in single generative factors, while being relatively invariant to changes in other factors [4]. For example, a model trained on a dataset of 3D objects might learn independent latent units sensitive to single independent data generative factors, such as object identity, position, scale, lighting or colour, similar to an inverse graphics model [24]. A disentangled representation is therefore factorised and often interpretable, whereby different independent latent units learn to encode different independent ground-truth generative factors of variation in the data.
% ●	Composition in Image Domains. To join segments of disparate image sources into one cohesive output, early works use hand-designed features, such as Laplacian pyramids for seamless blending (Burt & Adelson, 1983). To automate this, Isola & Liu (2013) and Hays & Efros (2007) employ nearest-neighbor approaches for scene composition and completion. More recently, a number of deep network architectures have been developed for compositional tasks. For discriminative tasks, Tabernik et al. (2016) and Kortylewski et al. (2020) train CNNs with modified compositional architecture for purposes of model interpretability and reasoning about object occlusion in classification. For image synthesis, Mokady et al. (2019) and Press et al. (2020) use an autoencoder to encode, disentangle, and swap properties between two sets of images, while Shocher et al. (2020) proposes mixing images in deep feature space while training the generator. Rather than creating models specifically for the image composition or scene completion objective, we investigate the ability of a pre-trained generator to mix-and-match parts of its generated images. Related to our work, Besserve et al. (2018) estimates the modular structure of GANs by learning a casual model of latent representations, whereas we investigate the generator’s compositional properties using image inversion


% ●	Some work has observed the vector arithmetic property [31, 36]. Beyond that, this work provides a detailed analysis of the semantics encoded in the latent space from both the property of a single semantic and the disentanglement of multiple semantics. Some concurrent work also explores the latent semantics learned by GANs. Jahanian et al. [20] studies the steerability of GANs concerning camera motion and image color tone. Goetschalckx et al. [14] improves the memorability of the output image. Yang et al. [38] explores the hierarchical semantics in the deep generative representations for scene synthesis. Unlike them, we focus on facial attributes emerging in GANs for face synthesis and extend our method to real image manipulation.
% ●	Semantic face editing aims at manipulating facial attributes of a given image. Compared to unconditional GANs which can generate image arbitrarily, semantic editing expects the model to only change the target attribute but maintain other information of the input face
% ●	In recent years, Generative Adversarial Networks (GANs) have significantly advanced image synthesis, particularly on face images. State-of-the-art image generation methods have achieved high visual quality and fidelity, and can now generate images with phenomenal realism. Most notably, StyleGAN [22, 23] proposes a novel stylebased generator architecture and attains state-of-the-art visual quality on high-resolution images. Moreover, it has been demonstrated that it has a disentangled latent space, W [8, 39, 44], obtained from the initial latent space Z via a Multi-Layer Perceptron (MLP) mapping network, which may offer control and editing capabilities. Recently, numerous methods have shown competence in controlling StyleGAN’s latent space and performing meaningful manipulations in W [39, 18, 41, 14, 3].


% ●	To show this, we make use of a newly proposed Attribute Dependency metric. Finally, we demonstrate the applicability of StyleSpace controls to the manipulation of real images. Our findings pave the way to semantically meaningful and well-disentangled image manipulations via simple and intuitive interfaces.


% ●	A recent topic of interest is editing images using generative models. A number of works propose linear attribute vector editing directions to perform image manipulation operations (Goetschalckx et al., 2019; Jahanian et al., 2020; Shen et al., 2019; Kingma & Dhariwal, 2018; Karras et al., 2019a; Radford et al., 2015). It is also possible to identify concepts learned in the generator’s intermediate layers by clustering intermediate representations, either using segmentation labels (Bau et al., 2018) or unsupervised clustering (Collins et al., 2020), and change these representations to edit the desired concepts in the output image. Suzuki et al. (2018) use a spatial feature blending approach which mixes properties of target images in the intermediate feature space of a generator. On faces, editing can be achieved using a 3D parametric model to supervise the modification (Tewari et al., 2017; 2020). In our work, we do not require clusters or concepts in intermediate layers to be defined a priori, nor do we need distinct input and output domains for approximate collages and real images, as in image translation tasks (Zhu et al., 2017; Almahairi et al., 2018). Unlike image manipulation using semantic maps (Park et al., 2019; Gu et al., 2019b), our approach respects the style of the manipulation (e.g. the specific color of the sky), which is lost in the semantic map representation. Our method shares commonalities with Richardson et al. (2020), although we focus on investigating compositional properties rather than image-to-image translation. In our approach, we only require a single example of the approximate target property we want to modify and use regression into the latent space as a fast image prior to create a coherent output. This allows us to create edits that are not contingent on labelled concepts, and we do not need to modify or train the generator.



% Related work Disentangled 
% ●	Interpretable Object-Centric Visual Models. Inspired by the analysis-by-synthesis approach for visual perception discussed in cognitive science [44], recent work [3, 7, 11, 36] propose structured latent space models to explain and synthesize images as sets of constituent components which are individually represented using VAEs [19] or GANs [10]. Other approaches favor explicit symbolic representations over distributed ones when parsing an image [33, 40] or propose probabilistic programming languages to formalize image generation [23]. In both cases, object-centric modeling allows decomposition of images into components and also enables targeted image modification via interpolation in symbol or latent space, e.g., altering position or color of an object parsed by the model. Interpretable and controllable factors of image generation are desirable properties for neural rendering models and have been investigated in recent image generation models, e.g., [1, 25, 28, 29]. However, despite the modeling effort put into the object representations, inter-object interactions are typically only modeled in a less explicit way, e.g., via image layers [36, 40], depth ordering variables [1] or an autoregressive scene prior [7]. Our work adds to this line of work by proposing a spatial correlation network which facilitates disentanglement of learned object representations and can be trained from raw observations.
% ●	recent work on compositional generative scene models [16, 17, 24–27, 38–44]
% ●	In all these methods, disentanglement is sought in latent space, with no grounding on the domain where the data is defined. For the case of images, we would like the independent factors to correspond to compact and simply-connected regions of the image, corresponding to objects. In all these methods, manipulation of the independent factors typically has global effects on the image, rather than enabling manipulation of one object at a time. We would like to develop models that naturally disentangle the spatial domain, in addition to other latent factors of variation.

% ●	Interpretable Object-Centric Visual Models. Inspired by the analysis-by-synthesis approach for visual perception discussed in cognitive science [44], recent work [3, 7, 11, 36] propose structured latent space models to explain and synthesize images as sets of constituent components which are individually represented using VAEs [19] or GANs [10]. Other approaches favor explicit symbolic representations over distributed ones when parsing an image [33, 40] or propose probabilistic programming languages to formalize image generation [23]. In both cases, object-centric modeling allows decomposition of images into components and also enables targeted image modification via interpolation in symbol or latent space, e.g., altering position or color of an object parsed by the model. Interpretable and controllable factors of image generation are desirable properties for neural rendering models and have been investigated in recent image generation models, e.g., [1, 25, 28, 29]. However, despite the modeling effort put into the object representations, inter-object interactions are typically only modeled in a less explicit way, e.g., via image layers [36, 40], depth ordering variables [1] or an autoregressive scene prior [7]. Our work adds to this line of work by proposing a spatial correlation network which facilitates disentanglement of learned object representations and can be trained from raw observations.

% ●	Experiments show that InfoGAN learns interpretable representations that are competitive with representations learned by existing supervised methods.
% ●	Unsupervised learning can be described as the general problem of extracting value from unlabelled data which exists in vast quantities. A popular framework for unsupervised learning is that of representation learning [1, 2], whose goal is to use unlabelled data to learn a representation that exposes important semantic features as easily decodable factors. A method that can learn such representations is likely to exist [2], and to be useful for many downstream tasks which include classification, regression, visualization, and policy learning in reinforcement learning. While unsupervised learning is ill-posed because the relevant downstream tasks are unknown at training time, a disentangled representation, one which explicitly represents the salient attributes of a data instance, should be helpful for the relevant but unknown tasks. For example, for a dataset of faces, a useful disentangled representation may allocate a separate set of dimensions for each of the following attributes: facial expression, eye color, hairstyle, presence or absence of eyeglasses, and the identity of the corresponding person. A disentangled representation can be useful for natural tasks that require knowledge of the salient attributes of the data, which include tasks like face recognition and object recognition. It is not the case for unnatural supervised tasks, where the goal could be, for example, to determine whether the number of red pixels in an image is even or odd. Thus, to be useful, an unsupervised learning algorithm must in effect correctly guess the likely set of downstream classification tasks without being directly exposed to them. A significant fraction of unsupervised learning research is driven by generative modelling. It is motivated by the belief that the ability to synthesize, or “create” the observed data entails some form of understanding, and it is hoped that a good generative model will automatically learn a disentangled representation, even though it is easy to construct perfect generative models with arbitrarily bad representations. The most prominent generative models are the variational autoencoder (VAE) [3] and the generative adversarial network (GAN) [4]. In this paper, we present a simple modification to the generative adversarial network objective that encourages it to learn interpretable and meaningful representations.
% ●	plays a pivotal role in disentangling the constituent components of a visual scene
% ●	Assuming a single observation or view x 1 for now, we can formally describe the goal of “multi-object” (i.e. object-centric) scene learning as that of computing the posterior p(z1, z2, ..., zK|x 1 ), where K is the number of 3D objects in the scene including the background “object”, zk ∈ R D is a D-dimensional latent representation of object k, and x 1 ∈ RM is a 2D image with M pixels. As K is unknown, recent “multi-object” works [4, 9] have fixed K globally to be a number that is sufficiently large (greater than actual number of objects) to capture all the objects in a scene and allowing for empty slots. Thus, we will use K to represent the number of object slots hereafter.
% ●	The contributions of the paper are as follows. First, we introduce a model that unifies the benefits of spatial-attention and scene-mixture approaches in a principled framework of probabilistic latent variable modeling. s makes the model applicable to scenes wת 
% ●	

% ●	To make sense of their visual environment, intelligent agents must construct an internal representation of the complex visual scenes in which they operate. Recently, one class of computer vision algorithms – Convolutional Neural Networks (CNNs) – has shown an impressive ability to extract useful categorical information from visual scenes. However, human perception (and the aim of computer vision) is not only about image classification. Humans also group scenes into object-centric representations in which information about objects, their constituent parts, positions, poses, 3D geometric and physical material properties, and their relationships to other objects, are explicitly available. Such object-centric, geometrically-rich representations natively build in key cognitive concepts such as object permanence, and naturally support high-level visual planning and inference tasks. 

% (e.g., the assignment of a fixed number of object slots per scene), and learn just from static images. 

%  Recent approaches from 3D computer vision, such as 3D-RelNet [29], have attacked the question from a different point of view, combining key geometric structures (such as meshes) with more standard convolutional features. Such works achieve effective results, but do not offer a solution when detailed supervision is unavailable. In this work, we propose a new representation, which we term Physical Scene Graphs (PSGs). The PSG concept generalizes ideas from both the MONet/IODINE and the 3D-RelNet 
 %  ****** lines of work, seeking to be at the same time geometrically rich enough to handle complex object shapes and textures, explicit enough about objects to support the top-down inferential reasoning capacities of generative models, flexible enough to learn from real-world or realistic (not toy) visual data,  % and self-supervisable, so as to not require extensive and laborious scene component labeling.
% ●	Image Synthesis: Generative Adversarial Networks (GANs) [16, 51] have significantly advanced the state-of-the-art in photorealistic image synthesis. In order to make the image synthesis process more controllable, several recent works have proposed to disentangle the underlying factors of variation [9, 25, 28, 41, 54, 74]. However, all of these methods ignore the fact that 2D images are obtained as projections of the 3D world. While some of the methods demonstrate that the disentangled factors capture 3D properties to some extend [9, 28, 41], modeling the image manifold using 2D convolutional networks remains a difficult task, in particular when seeking representations that faithfully disentangle viewpoint variations from object appearance and identity. Instead of directly modeling the 2D image manifold, we therefore follow a recent line of works [19, 30, 39] which aims at generating 3D representations and explicitly models the image formation process.
% ●	In this paper we have introduced an end-to-end method for generating diverse images from layout (bounding boxes + categories). Our method can generate reasonable images which look realistic and contain recognizable objects at the desired locations. We also showed that we can control the image generation process by adding/moving objects in the layout easily Moreover, making the image generation process more controllable, such as specifying the fine-grained attributes of instances, would be an interesting future direction.

% ●	We begin with the hypothesis that a model must be able to understand individual objects and relationships between objects in order to generate complex scenes with multiple objects well. Our layout-to-image-generation method, which we call Object-Centric Generative Adversarial Network (or OC-GAN), Introduction Generative Adversarial Networks (GANs) (Goodfellow et al. 2014) have been at the helm of significant recent advances in image generation (Goodfellow et al. 2014; Radford, Metz, and Chintala 2016; Gulrajani et al. 2017; Miyato and Koyama 2018; Brock, Donahue, and Simonyan 2019). Apart from unsupervised image generation, GAN-based image generation approaches have done well at conditional image generation from labels (Radford, Metz, and Chintala 2016; Zhang et al. 2019; Brock, Donahue, and Simonyan 2019), captions (Reed et al. 2016; Zhang et al. 2017; Xu et al. 2018b; Li et al. 2019a; Yin et al. 2019), conversations (Sharma et al. 2018; El-Nouby et al. 2019; Li et al. 2019b), scene graphs (Johnson, Gupta, and Fei-Fei 2018; Mittal et al. 2019; Ashual and Wolf 2019), layouts (Zhao et al. 2019; Sun and Wu 2019), segmentation masks (Park et al. 2019), etc. While the success in single-domain o
% ●	because they have many constituent objects (e.g., the Visual Genome dataset, Krishna et al. 2017, can contain as many as 30 different objects in an image). Past methods focus on different input types, including scene graphs (Johnson, Gupta, and Fei-Fei 2018; Ashual and Wolf 2019), pixel-level semantic segmentation (Li et al. 2019a), and bounding boxlevel segmentation (Zhao et al. 2019; Sun and Wu 2019). In addition, some methods also consider multi-modal data, such as instance segmentation alongside pixel-wise semantic segmentation masks (Park et al. 2019; Wang et al. 2018). Orthogonal to input-related considerations, methods tend to rely on additional components to help with the complexity of scene generation, such as attention mechanisms (Xu et al. 2018b; Li et al. 2019a) and explicit disentanglement of objects from the background (Singh, Ojha, and Lee 2019). Despite these advances, models still struggle in creating realistic scenes.
% ●	Our MVAE builds on previous neural probabilistic generative models, especially variational autoencoders (VAEs) [6, 10]. The DC-IGN [7], beta-VAE [5], and InfoGAN [1] are extensions and alternatives that promote learning latent codes whose individual features are “disentangled” [14, 2], i.e. correlated exclusively with underlying axes in the data-generating process. Other work has developed attention mechanisms for sampling subsets of visual scenes [9, 4, 15], which promotes learned representations that are spatially localized. Recurrent neural networks have been used in combination with spatial attention to allow for unsupervised learning of object locations and counts [3]. And several recent approaches allow object-like representations to be learned in supervised settings for visual question-answering and physical prediction [12, 16]. Another related strand of work focuses on explicit representations of multiple objects in visual scenes, making use of graphics engines as a known decoding function
% ●	SceneFID metric (FID per class ) (Object-Centric Image Generation from Layouts)
% ●	Scene-graphs and image matching Scene graphs are an object-centric representation that can provide an additional useful learning signal when dealing with complex scenes. Scene-graphs are often used as intermediate representations in image captioning (Yang et al. 2019; Anderson et al. 2016), reconstruction (Gu et al. 2019) and retrieval (Johnson et al. 2015), as well as in sentence to scene graph (Schuster et al. 2015) and image to scene graph prediction (Lu et al. 2016; Newell and Deng 2017). By virtue of being a simpler abstraction of the scene than a layout, they emphasize instance awareness more than layouts which focus on pixel-level class labels. Secondly, for scenarios that might require generating multiple diverse images, they provide more variability in reconstruction and matching tasks as the mapping from a scene graph to an image is one to many usually. These points explain their use in higher-level visual reasoning tasks such as visual question answering  etc.) from given spatial layouts and leverage them to learn the relationships between objects, which would be more difficult for a model to distill from pixel-level layouts.
% ●	Layout-based synthesis Generating images from a given layout makes the analysis more interpretable by decoupling the language understanding problem from the image generation task. Another advantage of generating from layouts is more controllable generation: it is easy to design interfaces to manipulate layouts. In this work we will focus on coarse layouts Finally, modulating the parameters of batch- or instance-normalization layers (Ioffe and Szegedy 2015; Ulyanov, Vedaldi, and Lempitsky 2016) with a function of the input condition can provide significant gains, and this is done per-channel in (Odena, Olah, and Shlens 2017) or per pixel (Park et al. 2019; Sun and Wu 2019). 
% ●	Abstract—With the remarkable recent progress on learning deep generative models, it becomes increasingly interesting to develop models for controllable image synthesis from reconfigurable inputs. This paper focuses on a recent emerged task, layout-to-image, to learn generative models that are capable of synthesizing photo-realistic images from spatial layout
% ●	R EMARKABLE recent progress has been made on both unconditional and conditional image synthesis [1], [2], [3], [4], [5], [6], [7], [8]. The former aims to generate highfidelity images from some random latent codes/vectors (e.g., sampled from the standard multivariate Gaussian distribution). The latter needs to do so with given conditions satisfied in terms of some consistency metrics. The conditions may take many forms such as category labels [3], [9], paired or unpaired source images [10], [11], [12], [13], semantic maps [14], [15], text description [16], [17] and scene graphs [18], [19]. C
% ●	Spatial layouts are usually used as intermediate representations for other conditional image synthesis tasks such as text-to-image [17], [21] and scene-graph-toimage [18], [19].

% ●	In addition to realness, generative models for layout-to-image need to tackle many spatial and semantic relationships among multiple objects (combinatorial in general). Specifically, learning layout-to-image requires addressing the problems of learning one-to-many mapping (i.e., one layout covers many plausible realizations in image synthesis to preserve the intrinsic uncertainty), and of handling consistent multi-object generation – the model can preserve the intrinsic one-to-many mapping from a given layout to multiple plausible images with sufficiently different structural and appearance styles 
% ●	both image and object levels, and (ii) Layout Control – the model is also adaptive with respect to changes of layouts (e.g., adding new objects), or perturbations of bounding boxes in a given layout, as well as the styles associated with the changes of spatial layouts. Prior arts on layout-to-image mainly focus on low resolution (64×64) [18], [20], except for the very recent Grid2Im method [19] which can synthesize images at a resolution of 256 × 256. Main drawbacks of existing methods are in two-fold: the diversity of styles in generated images is not sufficiently high to preserve the intrinsic one-to-many mapping for a given layout, and the controllability of styles along consecutive layout changes is often not sufficiently strong
% Our work is also related to image-to-image translation [13, 21], which translates a possible representation of an image into another representation. ●	

% Besides GAN-based approaches, CRN [3] used a cascaded refinement network with regression loss as training supervisions. SIMS [26] developed a semi-parametric approach, by retrieving fragments and refining them with a refinement network.



% ●	Interpretable directions in the latent space. Since the appearance of earlier GAN models, it is known that the GAN latent space often possesses semantically meaningful vector space arithmetic, e.g., there are directions corresponding to adding smiles or glasses for face image data (Radford et al., 2015). Since exploitation of these directions would make image editing more straightforward, the discovery of such directions currently receives much research attention. A line of recent works
% ●	on the model interpretability aims to train generators with disentangled latent spaces (Chen et al., 2016; Higgins et al., 2017; Liu et al., 2019; Lee et al., 2020; Ramesh et al., 2018). In particular, the seminal InfoGAN model (Chen et al., 2016) enforces the generated images to preserve information about the latent code coordinates by maximizing the corresponding mutual information. Another notable work proposes the β-VAE (Higgins et al., 2017) model, which puts more emphasis on the KL-term in the standard VAE’s ELBO objective. This objective modification requires the latent codes to be more “efficient”, which is shown to result in disentangled representations.
% ●	Disentanglement learning. An alternative line of research
% ●	In contrast, our method does not affect the pretrained generator distribution.
% ●	Recent works on generating high resolution images using generative adversarial networks (GANs) [18] have demonstrated the ability to generate photorealistic faces of novel identities, indistinguishable from real human faces [26, 28, 29]. However, these methods alone lack in terpretability and control over the outcome of the generative process as compared to the 3D graphic alternatives.
% ●	deepmind , invariances
% ●	distill simpler representation
% ●	(Isolating Sources of Disentanglement in VAEs) Learning disentangled representations without supervision is a difficult open problem. Disentangled variables are generally considered to contain interpretable semantic information and reflect separate factors of variation in the data. 

% ●	Unsupervised learning of disentangled representations is inherently a difficult problem due to the lack of a prior for semantic awareness, but we show some evidence in simple datasets with uniform factors that independence between latent variables can be strongly related to disentanglement.


% ●	(layoutVAE) Scene generation, which usually consists of realistic generation of multiple objects under a semantic layout, remains one of the core frontiers of computer vision. Despite the rapid progress and recent successes in object generation (e.g., celebrity face, animals, etc.) [1, 9, 13] and scene generation [4, 11, 12, 19, 22, 30, 31], little attention has been paid to frameworks designed for stochastic semantic layout generation. Having a robust model for layout generation will not only allow us to generate reliable scene layouts, but also provide priors and means to infer latent relationships between objects, advancing progress in the scene understanding domain.
% ●	Disentangled Representations. Many papers [2, 3, 5, 21, 22, 24, 26, 29] have tried to learn disentangled representations as part of image generation. Disentangled representations model different factors of data variations, such as class-related and class-independent parts [3, 21, 22, 26, 29]. By manipulating the disentangled representations, images with different appearances can be generated easily. In [24], three factors (foreground, background and pose) are disentangled explicitly when generating person image.
% ●	Latent Space Embedding With the rapid evolution of GANs, many works have tried to understand and control their latent space.
% ●	Compositional models. Compositional models have existed since the early days of computer vision [24] and have appeared mainly in two different varieties. The first flavor focuses on the creation of hierarchical feature representations by means of statistical modeling [8, 27, 48, 47], reusable deformable parts [49, 29], or compositional graph structures [36, 45]. The second flavor designs neural network-based representations in the form of recursive neural networks [38], imposing hierarchical priors on Deep Boltzman Machines [34], or introducing parametric network units that are themselves compositional [43]. The basis for our work is a notion of compositi
% ●	In fact, the effectiveness of deep learning is often ascribed to the ability of deep networks to learn representations that are insensitive (invariant) to nuisances such as translations, rotations, occlusions, and also “disentangled,” that is, separating factors in the high-dimensional space of data (Bengio, 2009).
% ●	We have shown that StyleSpace is highly disentangled, and proposed simple methods for detecting meaningful manipulation controls in this space. Future work should focus on finding meaningful control directions that involve multiple style channels. We also plan to develop inversion techniques that can deliver both high reconstruction accuracy and manipulability.
% ●	Visualizing deep neural networks. Various methods have been developed to understand the internal representations of networks, such as visualizations for CNNs (Zeiler & Fergus, 2014) and RNNs (Karpathy et al., 2016; Strobelt et al., 2018). We can visualize a CNN by locating and reconstructing salient image features (Simonyan et al., 2014; Mahendran & Vedaldi, 2015) or by mining patches that maximize hidden layers’ activations (Zeiler & Fergus, 2014), or we can synthesize input images to invert a feature layer (Dosovitskiy & Brox, 2016). Alternately, we can identify the semantics of each unit (Zhou et al., 2015; Bau et al., 2017; Zhou et al., 2018a) by measuring agreement between unit activations and object segmentation masks. Visualization of an RNN has also revealed interpretable units that track long-range dependencies (Karpathy et al., 2016). Most previous work on network visualization has focused on networks trained for classification; our work explores deep generative models trained for image generation.


% Related work GAN editing 


%%%%% Related Disen

% implicit understanding of structure or 
% 
% , but stills 
% However, these findings suggest  
% mostly global controllability, failing to
% current models still fail to support interpretability or controllability of particular objects or entities. 
% these are mostly concerned with implicit underdstanding
% structural hierachy
% of the latent space
% directions:
% hierarchical semantics
% the GAN latent space often possesses semantically meaningful vector space arithmetic, e.g., there are directions discovery of such directions

% Recent studies have shown that GANs naturally learn to encode rich semantics within the latent space, thus changing the latent code leads to 

% ****************************************some signs 
% While some works investigated Don’t explicitly account for that 

% **study internal representations of GANs and whether they have developed implicit notions for objects and their semantic relations.
% semantic hierarchy emerges as variation factors from synthesizing scenes from the generative representations
% determine the spatial layout and configuration, render the scene attributes as well as color scheme, control the categorical objects

% what a GAN actually learns with respect to the latent space.
% further shows that some units from intermediate layers of the GAN generator are specialized to synthesize certain visual concepts, such as sofa and TV for living room generation

% many works investigate how factors of variation can be disentangled

% Radford et al. [31] first observes the vector arithmetic property in the latent space. A recent work [4] further shows that some units from intermediate layers of the GAN generator are specialized to synthesize certain visual concepts,

% By either adding or reducing the activations of these neurons, objects can be added, expanded, reduced or removed.\\\\

% numerous methods have shown competence in controlling StyleGAN’s latent space and performing meaningful manipulations in W [39, 18, 41, 14, 3].

% several works (Jahanian et al., 2020; Plumerault et al., 2020; Goetschalckx et al., 2019; Shen et al., 2019) aim to identify semantically meaningful directions, i.e., corresponding to humaninterpretable image transformations.

% A number of works propose linear attribute vector editing directions to perform image manipulation operations

% Interpolations in latent space Traditional approaches to image editing with GAN latent spaces find linear directions that correspond to changes in labeled attributes,

% GAN dissection

% identify semantically meaningful directions, i.e., corresponding to humaninterpretable image transformations.
% attracted considerable attention
% controllable manipulation

% utilized semantic segmentation to analyze Progressive GAN [16] and detect causal units that control the presence of certain objects through ablation. Shen et al. [31] and Yang et al. [35] utilize classifiers to analyze StyleGAN [17] and show that a linear manipulation in W space can control a specific target attribute.

% However, most work focuses on property disentanglement, such as shape, pose and appearance, without considering the compositionality of the images, i.e., scenes being made up of multiple objects. Therefore, they do not offer control over individual objects in a way that respects the interaction of objects,
% This is a major limitation

% However, the obtained representation is often limited to a single object, hard to interpret As a result, these deep generative models cannot support manipulation tasks such as moving an object around
% computer graphic engines  often intuitive for scene manipulation.

% 
% but how GANs convert an unstructured latent code to a high quality output is still an open question.
% Yet in general, visual scenes contain a variable number of objects arranged in various spatial configurations, and often with partial occlusions (e.g., CLEVR, Johnson et al. 2017; see Figure 1). This motivates the question: 

% *****what forms a good representation of a scene with multiple objects? In line with recent advances 

%  , and can now generate images with phenomenal realism

%Image generation techniques based on GANs [3] are constantly improving in resolution, visual quality, the diversity of generated images, and the ability to cover the entire visual domain presented during training.

% Recently, unconditional generative adversarial networks (Karras et al., 2017; 2019b;a; Radford et al., 2015) have become capable of mimicking the complexity of natural images by learning a mapping from a latent space noise distribution to the image manifold. But how does this seemingly unstructured latent space produce a strikingly realistic and structured scene? 

% Convolutional generative adversarial networks have demonstrated impressive results in synthesizing high-resolution images [6, 26, 34, 53] from unstructured image collections. 

% The Significant strides have been made on generative models for image synthesis, with a variety of methods based on Generative Adversarial Networks (GANs) [14] achieving state-of-the-art performance.

% In recent years, Generative Adversarial Networks (GANs) have significantly advanced image synthesis, particularly on face images. State-of-the-art image generation methods have achieved high visual quality and fidelity, and can now generate images with phenomenal realism.

% The whirlwind of progress in deep learning has produced a steady stream of promising generative models [Goodfellow et al. 2014; Karras et al. 2018] that render natural scenes increasingly indistinguishable from reality and provide an intuitive way to generate realistic imagery given high-level user inputs [Bau et al. 2019; Wang et al. 2018].

% In recent years, the computer vision community has made great strides towards highly-realistic image generation. In particular, Generative Adversarial Networks (GANs) [24] emerged as a powerful class of generative models.

% In recent years, Generative Adversarial Networks have become ubiquitous in both research and public perception, 

% but:

% However, despite this success, state-of-the-art models struggle to properly disentangle the underlying generative factors

% but how GANs convert an unstructured latent code to a high quality output is still an open question.

% Yet in general, visual scenes contain a variable number of objects arranged in various spatial configurations, and often with partial occlusions (e.g., CLEVR, Johnson et al. 2017; see Figure 1). This motivates the question: 

% what forms a good representation of a scene with multiple objects? In line with recent advances 

% high visual quality and fidelity , and can now generate images with phenomenal realism

% Image generation techniques based on GANs [3] are constantly improving in resolution, visual quality, the diversity of generated images, and the ability to cover the entire visual domain presented during training.

% However, most work focuses on property disentanglement, such as shape, pose and appearance, without considering the compositionality of the images, i.e., scenes being made up of multiple objects. Therefore, they do not offer control over individual objects in a way that respects the interaction of objects,
% This is a major limitation

% However, the obtained representation is often limited to a single object, hard to interpret As a result, these deep generative models cannot support manipulation tasks such as moving an object around
% computer graphic engines  often intuitive for scene manipulation.





% ***we follow the philosophy proposed/introduced by this line of work and marry its merits incoporate this into the generative adversarial framework. 


% ______________________
% Disentangled: 
% ***marry
% Letting explicit control into this multi-stage / iterative process. Iterative by semantic decomposition rather than solely visual depcompostiion
% To the extent that would like to capture the compositionality of the scenes.

% Recent work, such as MONet [4] and IODINE [17], has made initial progress in attempting to 
%  Learning from self-supervision with visual data, these works achieve some success at . However, these approaches are limited by architectural choices As a result, they do not generalize effectively to complex real-world image data.

% given an input scene 

% inferring latent representations for simple synthetic scenes
% Sequential models have been pivotal for improved image generation using variational autoencoders:
% ___

% Draw, IODINE scene decomposition, VAE models like MONet and IODINE give iterative/compositional generation 

% IODINE [13] also employs a spatial mixture model to jointly infer the segmentation and object representation. 

% Eslami et al., 2016; Kosiorek et al., 2018 use an iterative procedure to infer a variable number of latent variables, one for every object in a scene, that are highly informative of the object class, while Greff et al., 2019; Burgess et al., 2019 perform unsupervised instance-level segmentation in an iterative fashion.

%  DRAW (Gregor et al., 2015) uses attention based recurrence conditioning on the canvas drawn so far. In Eslami et al. (2016), a recurrent generative model that draws one object at a time to the canvas was used as the decoder in VAE. 

% ___


% there is 
%%%  /given
% *** from simple 2d images
%  Drawing inspiration 

% but don’t scale well to images beyond simple 2d settings.
% do not generalize effectively to complex real-world image data.
% These methods are yet to show scalability to natural images.
% simulated datasets and not real images, simpler synthetic datasets
% [13] does not perform well on textured or cluttered scene, culprit the assumption that pixels can be grouped into objects according to the low dimensional spa
% ___

% **** generative adverserial networks

% ***************The recent GANsformer architecture \cite{gansformer} heads in the right direction, by leveraging soft-attention [mechanisms] for the task of image generation. In this work, we take a step further, and show how we can use the GANsformer approach as a backbone, and extend it to enable not only an implicit, but also an \textit{explicit modeling} of compositional scenes.
% ***************To this end, we leverage the recently introduced GANsformer \cite{gansformer} soft-attention architecture for image generation, and as will be discussed in detail in the next section, take it a step further so to enable not only an implicit, but also an \textit{explicit modeling} of compositional scenes.

% /push it a step 
% a more natural scene synthesis more closely how a human would approach producing . 

% Our work also fit into the wider family of two-stage generation.
% we go a step forward and leverge the ideas proposed by the GANsformer work, and use it as a backbone in a novel iterative model to enhance the compositionality of the generative process
% in contrast, 
% ** structural
% use it as a backbone that will 

% GANsformer is a step in the right direction but still doesn’t give full disentanglement.




% Prior works on incorporating inductive biases aimed at object compositionality typically treat an image as a spatial mixture of image patches and utilizes multiple copies of the same function to arrive at a compositional solution.

% ****In the real world, objects are not strictly independent of one another. Certain objects may only occur in the presence of others, or affect their visual appearance in subtle ways (eg. shadows). 


% Our work is also related to studies investigating the modularity and the composability of GANs [17, 53]. Recently, Zhao et al. [53] proposed a modular multidomain GAN architecture, which consists of several composable modular operations

% weak or strong full or partial mutual independence assumptions that doesn't translate to real scenes beyond CLEVR
% provides interpretable parameters for the scene,
% However, BlockGAN comes with a significant limitation in that it assumes that objects are mutually independent. incorporating concepts such as position and orientation
% acceptable only when objects interact weakly, but it is badly violated for medium to densely packed scenes, correlations or dependencies are strong

% ______________________
% iterative:

% Our work also holds relations. In contrast to early approaches, outperform, like us, employ a two-stage generation procedure, e.

% In S2 -GAN (Wang & Gupta, 2016), an image-to-image adversarial network takes a map of surface normal as condition and outputs another realistic image, where the normal map is generated by another vanilla GAN to represent the structure of a scene. By using an U-net generator and a convolutional discriminator, pix2pix model (Isola et al., 2017) performs well on a wider variety of image-to-image tasks, including style transferring and reconstructing images from label maps or edge maps.

% S2 -GAN [27] factorizes the image generation process into style and structure components. It combines two GANs, one for generating structure information, i.e. surface normals, and one for generating style information, i.e, appearance, where surface normals are used as a condition vector to generate indoor scenes.

% compose sequential ordered layers
% images are composed by combining different layers with different alpha masks.

% learn composable module operations which are able to either add or remove a particular ingredient

%   Early compelling results using GANs used sequential coarse-to-fine multiscale generation and classconditioning (Denton et al., 2015). 

% Zhang et al. [30] propose a GAN based image generation framework where the image is progressively generated in two stages at increasing resolutions

%  Various coarse-to-fine schemes [4] have been proposed [9,19,26,57] to synthesize larger images (e.g. 256 × 256) in an unconditional setting. Inspired by their successes, we propose a new coarse-to-fine generator and multi-scale discriminator architectures suitable for conditional image generation at a much higher resolution.

%  Gregor et al. [16] advocate for a recurrent approach for image generation, with successive rounds of refinement in a generative process that remains close to the pixels. A push toward hierarchical variants could include layers or successively more abstract information regarding image content.

% One closely related work combining recursive structure with GAN is that of Im et al. (2016) but it does not explicitly model object composition and follows a similar paradigm as by Gregor et al. (2015).

% Besides using a single GAN for generating images, there is also work [36, 5, 10] that utilized a series of GANs for image generation. Wang et al. [36] factorized the indoor scene generation process into structure generation and style generation with the proposed S 2 -GAN. In contrast, the second stage of our StackGAN aims to complete object details and correct defects of Stage-I results based on text descriptions. Denton et al. [5] built a series of GANs within a Laplacian pyramid framework. At each level of the pyramid, a residual image was generated conditioned on the image of the previous stage and then added back to the input image to produce the input for the next stage. Concurrent to our also showed that they can generate better images by stacking several GANs to reconstruct the multi-level representations of a pre-trained discriminative model. However, they only succeeded in generating 32×32 images, while our method utilizes a simpler architecture to generate 256×256 images with photo-realistic details and sixty-four times more pixels.

% The idea of inferring scene structure for image generation is not new, as it has been explored by some recent works in several domains. For example, Wang et al. [32] proposed to infer a surface normal map as an intermediate structure to generate indoor scene images, and Villegas et al. [29] predicted human joints for future frame prediction. The most relevant work to our method is Reed et al. [23], which predicted local key-points of bird or human for textto-image synthesis

% modeling section

% GAN learns to generate image background and foregrounds separately and recursively

% semantic layout a coarse-to-fine
% cascade of generative models, each of them captures the image structure at a particular scale of a Laplacian pyramid. Zhang, Xu, and Li improve the image quality by increasing image resolution with a two-stage GANs.
% adopt a layered structure modeling and compose a scene sequentially.
% LR-GAN learns to generate image background and foregrounds separately and recursively, and stitch the foregrounds on the background in a contextually relevant manner to produce a complete natural image. For each foreground, the model learns to generate its appearance, shape and pose.
% In [50], the authors use the concept of image layers and propose a layered GAN model that learns to generate background and foreground images separately and recursively and then compose them into a final composite image. 

% ___________________
% conditional:




% Other works, such as SPADE \citep{spade,sean}, employ region-based feature modulation for the task of layout-to-image translation, but, contrary to us, use fixed segmentation maps or static class embeddings to control the visual features. Of particular relevance is the prominent StyleGAN model \citep{stylegan,stylegan2}, which utilizes a single global style vector to consistently modulate the features of each layer. The GANsformer generalizes this design, as multiple style vectors impact different regions in the image concurrently, allowing for a spatially finer control over the generation process.

% ***directly comparable 

% Pix2pix [22] adopts a U-Net architecture to synthesize lowresolution images from a semantic map. To operate in high-resolution settings, Pix2pixHD [46] introduces the multi-scale generator and discriminator network structure to enhance the quality of the generated images. SPADE [35] further improves Pix2pixHD with the spatially-adaptive normalization layers. Different from 

% First, SPADE uses only one style code to control the entire style of an image, which is not sufficient for high quality synthesis or detailed control. does not allow using a different style input image for each region in the segmentation mask.
% Second, we believe that inserting style information only in the beginning of a network is not a good architecture choice. Recent architectures [26, 32, 2] have demonstrated that higher quality results can be obtained if style information is injected as normalization parameters in multiple layers in the network, e.g. using AdaIN [20]. However, none of these previous networks use style information to generate spatially varying normalization parameters. To alleviate this shortcoming, our second main idea is to design a normalization building block, called SEAN, that can use styleinput images to create spatially varying normalization parameters per semantic region. An important aspect of this work is that the spatially varying normalization parameters are dependent on the segmentation mask as well as the style input images.

% conditional image synthesis that aims at generating photo-realistic images conditioned on input segmentation masks, which is called semantic image synthesis

% seminal U-net SPADE proposes a spatial-varying normalization layer for the first time and has a profound impact as a basic backbone.

% Given a semantic label map, our approach produces an image with photographic appearance that conforms to the input layout.

% [36] propose a spatiallyadaptive normalization for synthesizing photo-realistic images given an input semantic map. With the useful semantic information, existing methods on both tasks achieved promising performance in scene generation.

%  Several recent studies have demonstrated the potential of variant GANs for scenelevel complex image generation from text [37, 20], scene graph [23], semantic layout map [20, 38].
 
% Conditional GANs (cGANs) are able to generate an output image conditioned on an input image. This makes these models suitable for solving image-to-image translation tasks where an image from one specific domain is translated into another domain. Several image-to-image translation approaches based on cGANs have been proposed [5, 8, 22, 23, 31, 34, 47, 55, 56]. Isola et al. [23] proposed a generic image-to-image translation approach using cGANs trained with a set of aligned training images from the two domains. CycleGAN [55] bypasses the need of aligned pairs of training samples by introducing a cycle consistency loss that prevents the two generators from contradicting each other and alleviates the mode collapse problem of GANs. 
% seminal

% Semantic image synthesis. Pix2pix (Isola et al., 2017) first proposed to use conditional GANs (Mirza & Osindero, 2014) for semantic image synthesis, adopting an encoder-decoder generator which takes semantic label maps as input, and employing a PatchGAN discriminator. Since then, various generator and discriminator modifications have been introduced (Wang et al., 2018; Park et al., 2019; Liu et al., 2019; Tang et al., 2020c;b; Ntavelis et al., 2020). 

% Conditional image synthesis exists in many forms that differ in the type of input data. For example, class-conditional models [3, 36, 37, 39, 41] learn to synthesize images given category labels. Researchers have explored various models for generating images based on text [18,44,52,55]. Another widely-used form is image-to-image translation based on a type of conditional GANs converting segmentation masks to photorealistic images 

% These approaches condition the generation on various types of information. For example, [29,31,57,5] synthesize images characterized by a single label. In a different setting, [39,58,59,52] employ a text to image pipeline to create an image based on a high-level description. Recently, many methods utilize information of a scene graph [18,2] to represent where objects should be positioned on the output image. A more fine-grained approach aims to translate semantic maps, which carry pixel-wise information, to realistic looking images [14,47,35,22]. 

% We consider semantic image synthesis, which aims at generating photorealistic images conditioned on semantic layouts. 

% synthesizing photo-realistic images from ground truth segmentations

% A traditional GAN uses noise vectors as the input and thus provides little user control. This motivates the development of conditional GANs (cGANs) [36] where users can control the synthesis by feeding the generator with conditioning information. Examples include class labels [38, 35, 6], text [42, 19, 49]


% Conditional GANs [20] generate appealing images in a variety of applications including image to image translation both in the case of paired [10] and unpaired data [38, 39],

% ’pix2pix’[14] of Isola et al. uses a conditional GAN [10] to learn a mapping from input to output images. In CycleGAN [45], a cycle consistency loss is proposed to enforce one-to-one mapping.
% semantic layouts
% 
% One important class of CGANs use images as conditioning information, such as pix2pix (Isola et al. 2017), BicycleGAN (Zhu et al. 2017b), pix2pixHD (Wang et al. 2018),SPADE (Park et al. 2019), MaskGAN (Lee et al. 2019) and SEAN (Zhu et al. 2019a)

% Image-to-Image Image-to-Image translation techniques aim at learning a conditional image generation function that maps an input image of a source domain to a corresponding image of a target domain. Isola et al. [17] first introduced the use of conditional GANs to solve various image-toimage translation tasks.

% Wang and Gupta [47] synthesize 128×128 images of indoor scenes by factorizing the image generation process into synthesis of a normal map and subsequent synthesis of a corresponding color image.

% either feed the semantic label maps as inputs to the generator, or use them to modulate the activations in normalization layers via affine transformations.

% Pix2pix [7] is a fully supervised method

% Conditional generation ultimately likewise relies on auto-encoding losses (feature matching / perceptual loss) that limit the image variation.

% one-to-many mapping

% Generative adversarial networks (GAN) [6] has made great success in image synthesis [1, 17, 22]. Conditional GANs synthesize images based on given conditions, which can be labels [34, 1], sentence descriptions [33, 31], or semantic layout in our task.  Semantic image synthesis aims at synthesizing photorealistic images given the semantic layout. Pix2pix [13] adopted an encoder-decoder generator which takes semantic label maps as inputs. Pix2pixHD [29] proposed a coarse-to-fine generator and multi-scale discriminators to generate high-resolution images. SPADE [25] used the semantic label maps to predict affine transformation parameters for modulating the activations in normalization layers. 

% regression loss

% ______________________
% non multi:
% However, most techniques in this space have focused on generating a single result. However, the quality has been attained at the expense of multimodality, as the generator learns to largely ignore the random noise vector when conditioned on a relevant context [20, 34, 40, 45, 47, 55]. In fact, it has even been shown that ignoring the noise leads to more stable training [20, 29, 34].

% For semantic image synthesis, the VGGbased perceptual loss was first introduced by CRN, and later adopted by Pix2pixHD. Since then, it has become a default for training the generator (Park et al., 2019; Liu et al., 2019; Tan et al., 2020; Tang et al., 2020a). We experimentally show that such loss imposes unnecessary constraints on the generator, significantly limiting sample diversity. While our model, trained without the VGG loss, achieves improved image diversity while not compromising image quality.

% L1 or l2 features pixel or loss 

% ______________________
% advtanges:
% both require traning, but only their conditional
% A key practical drawback of such conditional models is that they require full segmentation layouts as input. Thus, unlike unconditional generative approaches which synthesize images from randomly sampled noise, these models are limited to generating images from a set of scenes that is prescribed in advance, typically either through segmentation labels from an existing dataset, or scenes that are hand-crafted by experts. 
% perceptual feature reconstruction
% ______________________
% text:


% bound 
% and generally-applic
% while offering a more 

% heavy-engineed pipelines with multiple stages and forms of inputs and supervision including text or scene graphs, boundings boxes, segments and a ground-truth image.
% pipeline
% ***simpler design streamlined generallly applicable tied 
% unlike 

% Other recent work in GANs has focused on conditional image generation to simplify the task of multi-object image generation. Johnson et al. (2018) generate multi-object images from explicit scene graphs, while Xu et al. (2018) condition on a stochastic and-or graph instead. Azadi et al. (2019) propose a framework to generate images composed of two objects by combining the images of each individual object. Similarly, Lin et al. (2018) present an iterative scheme to remove or add objects to a scene based on prior knowledge about individual objects. Hinz et al. (2019) require object labels and bounding boxes to generate complex visual scenes consisting of multiple objects and background. While these works generate realistic multi-object scenes, they require prior information (scene graphs, segmentations, etc.) about individual objects or scenes that is typically not available in many real-world settings. while we consider visually simpler scenes,

% from language description

% The text-to-image synthesis model proposed in [17] decomposes the synthesis task into multiple steps. First, given the text description, a semantic layout is constructed by generating object bounding boxes and refining each box by estimating object shapes. Then, an image is synthesized conditioned on the generated semantic layout from the first step. Our work shares the same high-level idea A key difference is that we focus

% Hong et al. (2018b) use the image caption to generate bounding boxes of specific objects within the image and predict the object’s shape within each bounding box. 

% [9] proposes to decompose the generation process into two steps, in which it first constructs a semantic layout (bounding boxes and object shapes) from the text and then synthesizes an image conditioned on the layout and text description.

% Hong et al. [11] break down the process of generating an image from a sentence into multiple stages. The input sentence is first used to predict the objects that are present in the scene, followed by prediction of bounding boxes, then semantic segmentation masks, and finally the image

% In prior works, it is usually served as an intermediate representation between other input sources (e.g., text [11] or scene graphs [14]) In [11, 14], instead of learning a direct mapping from textual description/scene graph to an image, the generation process is decomposed into multiple individual steps. They first construct a semantic layout (bounding boxes + object shapes) from the input, and then convert it to an image using an image generator. % Both of them can generate an image from a coarse layout together with textual description/scene graph.\\
% ______________________
% editing: 
% propose linear attribute vector editing directions to perform image manipulation operations
% Scene manipulation and editing. 
% ***specialized optimization and inversion techniques per image 
% allowing to transform or edit a given image in various imaginative ways

% This editing scheme will allow users to manipulate a photograph not with physical colors, but with abstract concepts such as object types and visual attributes. 

% on object-level semantic editing, allowing users to interact with the entire scene and manipulate individual objects in the image

% most of demand heavy optimization method per each image 
% directly optimizing the latent code for an individual image

% none can move an object 
% ______________________
% composition: 
% pre-trained GAN to mix-and-match parts of its generated images

% Image composition aims to generate new images by embedding foreground objects into background images. It strives for synthesis realism by adjusting the size and orientation of the foreground objects as well as blending between foreground objects and background images.

% Composition in Image Domains. To join segments of disparate image sources into one cohesive output, blending  

% Image composition is a challenging problem in computer graphics where objects from different images are to be overlaid in one single image.
% process of overlaying a masked foreground image on top of a background image.
% Image inpainting

% ______________________
% depth ordering:
%More recently, Yang et al. [51] proposed a layered model for object detection and segmentation that estimates depth ordering and labeling of the image pixels. In [50], the authors use the concept of image layers and propose a layered GAN model that learns to generate background and foreground images separately and recursively and then compose them into a final composite image. 

% Several approaches have been also proposed for the amodal detection [25] or segmentation [15, 30, 57], the task of detecting or segmenting the full extent of an object including any invisible and occluded parts of it.

% ______________________
% model:

% In this work, we present a scene generation framework based on Generative Adversarial Networks (GANs) to sequentially compose a scene, breaking down the underlying problem into smaller ones. Different than the existing approaches, our framework offers an explicit control over the elements of a scene through separate background and foreground generators. Starting with an initially generated background, foreground objects then populate the scene one-by-one in a sequential manner. Via quantitative and qualitative experiments on a subset of the MS-COCO dataset, we show that our proposed framework produces not only more diverse images but also copes better with affine transformations and occlusion artifacts of foreground objects than its counterparts. Introduction The visual world we sense, interpret and interact everyday is a complex composition of interleaved physical entities. Scenes we perceive can then be altered due to accidental factors such as occlusions caused by inter-entity interactions and self-occlusions caused by differing vantage points with respect to the camera. These factors do not only make the problem harder but also diversifies the possible space of configurations given a fixed set of observable entities. Consequently, scene generation is challenged by high sample complexity in addition to photorealism constraints. Scene generation problem has been studied extensively in (Hertzmann et al. 2001; Tappan 2008; Chen et al. 2009; Isola and Liu 2013), however the interest has certainly expanded with the advent of Generative Adversarial Networks (GANs) (Goodfellow et al. 2014). Although recently there have been great strides in the quality and resolution of generated images (Miyato et al. 2018; Wang et al. 2018), it has mostly been addressed as learning a mapping from a single source, e.g. noise or semantic map, to target, e.g. images of giraffes, discarding almost all of the underlying complexity that forms a scene. This formulation sets two major restrictions on (i) ability to control scene elements, e.g. “What objects will appear?” or “How will they appear?”, (ii) ability to manipulate an existing scene, e.g. “Make that cow larger!”, while keeping rest of the scene unaltered. One possible explanation is that a single source representation such as a noise vector z is insufficient to explain all the complexity involved in describing a scene meaningfully. In this paper, we tackle the scene composition task with a layered structure modeling approach. This formulation helps reducing the complexity of the problem since we deal with one subproblem at a time. Furthermore, our framework allows for explicit control mechanisms at multiple levels such as scene layout and individual object appearances which lack in the previous approaches. Our main idea resembles how a landscape painter would first sketch out the overall structure, e.g. first a background such as mountain ranges or rivers, and later embellish the scene gradually with other elements to populate the scene, e.g. foreground instances such as trees and animals. Our proposed sequential framework works in an analogous manner to the procedure as depicted in Figure 1. It starts with a background generator to fill the canvas at the first time step. In every consecutive time step a foreground generator draws then a new entities conditioned on an instance mask and the canvas passed on from previous time step giving the user control over where and how the object will appear in the scene. Our model simultaneously aims to preserve the previously drawn background scene and added entities. We propose a novel image generation framework to sequentially compose a scene, element-by-element. We achieve this by an explicit control over the elements of a scene through separate background and foreground generators. This allows user control over the objects to generate, as well as, their category, their location, their shape and their appearance.


% In summary, we introduce a new architecture building block SEAN that has the following advantages: 1. SEAN improves the quality of the synthesized images for conditional GANs. We compared to the state of the art methods SPADE and Pix2PixHD and achieve clear improvements in quantitative metrics (e.g. FID score) and visual inspection. 2. SEAN improves the per-region style encoding, so that reconstructed images can be made more similar to the input style images as measured by PSNR and visual inspection. 3. SEAN allows the user to select a different style input image for each semantic region. This enables image editing capabilities producing much higher quality and providing better control than the current state-ofthe-art methods. Example image editing capabilities are interactive region by region style transfer and perregion style interpolation (See Figs. 1, 2, and 5).
% In this paper, we combine the merits of sequential generation with the flexibility of GANs. Our model for sequential generation imbibes a recursive structure that more naturally mimics image composition by inferring three components: appearance, shape, and pose. 
% Such scenes are composed of a variable number of objects, with individual properties and relations among them. Effective latent representations for these images need flexibility and compositionality.
% Moreover, the discriminator can also 

% modular, generalized, compositional representations for high-level concepts. learning of compositional, modular latent representations for scenes.

% Using this general design as a backbone
%  incorporate dependencies among objects and background in the generative process

% inally, we demonstrate how one can leverage the learned structured generative process, which is now interpretable and semantically understood,
% 

% visual scene into distinct parts, describe relations between them and reason about their dynamics They maintain explicit object representations,

% built-in inductive biases. This factored representation allows more flexibility in the generated scenes; In this paper, we combine the merits of sequential generation with the flexibility of GANs.

% compositionality: the notion that the representation of the whole should be composed of the representation of its parts

% Intuitively, encouraging this property during training results in representations that are more robust to re-combination (e.g., when seeing a familiar object in a novel context) and less prone to focusing on discriminative but irrelevant background features

% Semantic layout defines a structure of scene based on object instances and provides fine-grained information of the scene, such as the number of objects, object category, location, size, shape, etc.

% To address this issue, we propose a novel deep structured generative model which boosts generative adversarial networks (GANs) 

% To the extent that the scene is compositional, one could change the style, color or material of one object without necessarily changing its context. 

% Definitions of disentanglement vary [5, 52], but commonly refer to being able to control an attribute of interest, e.g. object shape, size, or pose, without changing other attributes. 
% a structural loss function to evaluate
% network architecture, training objective
% from scratch
% conditioned on that layout

% , we draw inspiration from the scene descomposition literature: 

% *****
% *to enhance the compositionality of the generative process
% ************intermediate representations


% ***
% ***decompose a visual scene into its constituent components and to generate a (learned) number of latent variables that explicitly encode the location and appearance of each object coherent regions
% *

% adopts
% a one-to-many mapping
% **techniques
% hence
% condition 
% favourable
% [stackGAN, progan] yield outperforms
% guide the process,

% ****contemporary 
% **Our work is inspired by prior work on obtaining interpretable visual representations with neural networks

% The proposed SAGAN performs better than prior work1 , boosting the best published Inception score from 36.8 to 52.52 and reducing Frechet Inception distance from 27.62 to ´ 18.65 on the challenging ImageNet dataset

% Empirically, we provide an extensive evaluation of our method on several challenging datasets: CelebAMaskHQ [29, 25, 33], CityScapes [10], ADE20K [53], and our own Fac¸ades dataset. Quantitatively, we evaluate our work on a wide range of metrics including FID, PSNR, RMSE and segmentation performance; qualitatively, we show examples of synthesized images that can be evaluated by visual inspection. Our experimental results demonstrate a large improvement over the current state-of-the-art methods. 
% ______

% ***************Realistic visual scenes contain rich structure, which humans effortlessly exploit to reason effectively and intelligently.

% ********************The ability to decompose complex multi-object scenes into meaningful abstractions like objects is fundamental to achieve higher-level cognition. factorized object representations

% The visual world we sense, interpret and interact everyday is a complex composition of interleaved physical entities.

% manipulating the corresponding attributes of the output images 

% Of particular practical importance are controls that are interpretable and disentangled, as they suggest intuitive image manipulation interfaces.

% In this study, we aim to , to this end, we propose, 

% Our key hypothesis is that incorporating a compositional 3D scene representation into the generative model leads to more controllable image synthesis.

% Meanwhile, sketches are easily editable: such an advantage is further amplified by the increasing popularity of touch-screen devices. Sketching thus becomes one of the most important ways that people illustrate their ideas and interact with devices

% Empirical evaluation shows that our Semantic Bottleneck GAN achieves a new state-of-the-art on two complex datasets, Cityscapes and ADE-Indoor, as measured both by the Frechet Inception Distance (FID) and by ´ user studies. Additionally, we observe that the synthesized segmentation label maps produced as part of the end-toend image synthesis process in Semantic Bottleneck GAN can also be used to improve the performance of the stateof-the-art semantic image synthesis network [32], resulting in higher-quality outputs when conditioning on ground truth segmentation layouts. 

% s. It demonstrates that the attention mechanism gives more power to both the generator and the discriminator to directly model the long-range dependencies in the feature maps. In addition, the comparison of our SAGAN and the baseline model without attention (2nd column of Table 1) further shows the effectiveness of the proposed self-attention mechanism



% Modelling 
% ●	Train on oasis, + nice regularization Semantic matching loss but cuts loss better for the unserupvsied case where we dont have classes + shared trunk of 256-> 16 for computational efficiency Hypothesis that semantic matching may lead to typical less varied textures as well as less variance in the object arrangements so to each the task of the segmenter component within the discriminator. Essentially, we would like the image to looks realistic, rather than necessarily to allow to easy segmentation easy-to-segment  - heavier disbinirator computationally 
% ●	(DO 2D GANS KNOW 3D SHAPE? UNSUPERVISED 3D) Through our investigation, we found that such a pre-trained GAN indeed contains rich 3D knowledge and thus can be used to recover 3D shape from a single 2D image in an unsupervised manner. The core of our framework
% ●	Perceptual Reconstruction loss to enforce consistency or other forms of supervised signals entailed from the paired nature of input-outputs  availability of 
% ●	. Adding additional ‘patch discriminators’ (Isola et al., 2017), where patches correspond to objects may serve a starting point in pursuing this direction. (compGAN)

% Conditional disentanglement 
% ●	Conditionally independent disentanglement
% ●	Having a cup and a plate on a desk. Cup and plate positions can be considered largely/mostly independent of each other but not independent of the desk position. And beyond position correlation the fact that no two objects can occupy the same position also means they are all dependent on each other.
●	Recent studies of disentangled representations [8, 28] consider a latent representation to be perfectly disentangled if each latent dimension controls a single visual attribute (disentanglement), and each attribute is controlled by a single dimension (completeness).
●	A disentangled representation can be defined as one where single latent units are sensitive to changes in single generative factors, while being relatively invariant to changes in other factors [4]. For example, a model trained on a dataset of 3D objects might learn independent latent units sensitive to single independent data generative factors, such as object identity, position, scale, lighting or colour, similar to an inverse graphics model A disentangled representation is therefore factorised and often interpretable, whereby different independent latent units learn to encode different independent ground-truth generative factors of variation in the data. 
●	Humans can understand unfamiliar circumstances quickly. For the scene shown in Figure 1, one can recover the shape of the sofa though some parts of it are occluded by clothes. To endow agents with this basic but important capability,
●	most work focuses on property disentanglement, such as shape, pose and appearance, without considering the compositionality of the images, i.e., scenes being made up of multiple objects. Therefore, they do not offer control over individual objects in a way that respects the interaction of objects, such as consistent lighting and shadows. This is a major limitation of current image generative models, compared to the graphics pipeline, where 3D objects are modelled individually in terms of geometry and appearance, and combined into 3D scenes with consistent lighting.



●	Even when considering object compositionality, most approaches treat objects as 2D layers combined using alpha compositing [14, 53, 56]. Moreover, they also assume that each object’s appearance is independent [4, 8, 14]. ance interactions between objects, such as scene lighting that affects objects’ shadows on a background.
●	Amodal completion
●	l relational learning models [28, 48, 54] (Transformers, RNs, contrastive world)
●	The key idea behind the unsupervised learning of disentangled representations is that real-world data is generated by a few explanatory factors of variation which can be recovered by unsupervised learning algorithms. 






●	There are various definitions for disentanglement [54, 50, 2, 7, 19], but a common goal is a latent space that consists of linear subspaces, each of which controls one factor of variation. However, the sampling probability of each combination of factors in Z needs to match the corresponding density in the training data. As illustrated in Figure 6, this precludes the factors from being fully disentangled with typical datasets and input latent distributions.2
●	our investigations to the separation of high-level attributes and stochastic effects, as well as the linearity of the intermediate latent space will prove fruitful in improving the understanding and controllability of GAN synthesis.
●	. In general, we expect that methods for directly shaping the intermediate latent space during training will provide interesting avenues for future work
●	While there is no single formalized notion of disentanglement (yet) which is widely accepted, the key intuition is that a disentangled representation should separate the distinct, informative factors of variations in the data (Bengio et al., 2013). A change in a single underlying factor of variation zi should lead to a change in a single factor in the learned representation r(x). 
●	Conditional disentanglement rather than independence Consider the commonly used “intuitive” notion of disentanglement which advocates that a change in a single groundtruth factor should lead to a single change in the representation. intervention
●	To gain a conceptual understanding of our world, models must first learn to understand the factorial structure of low-level sensory input without supervision (Bengio et al., 2013; Lake et al., 2016; Higgins et al., 2017). As argued in several notable works (Desjardins et al., 2012; Bengio et al., 2013; Chen et al., 2016; Higgins et al., 2017), this understanding can only be gained if the model learns to disentangle the underlying explanatory factors hidden in unlabelled input. A disentangled representation is generally described as one which separates the factors of variation, explicitly representing the important attributes of the data (Desjardins et al., 2012; Bengio et al., 2013; Cohen & Welling, 2014b; Kulkarni et al., 2015; Chen et al., 2016; Higgins et al., 2017). For example, given an image dataset of human faces, a disentangled representation may consist of separate dimensions (or features) for the face size, hairstyle, eye colour, facial expression, etc
●	of a disentangled representation [Higgins et al., 2018, Locatello et al., 2018, Higgins et al., 2017a]. In this paper, when evaluating disentangled representations we both employ standard metrics [Kim and Mnih, 2017, Chen et al., 2018, Locatello et al., 2018] and (in view of their limitations) emphasize visualization analysis


●	• Improvements to both disentangling and reconstruction accuracy on datasets of simple objects. • Complementarity to (and improvement of) state-of-the-art disentangling techniques. • Particularly significant benefits when the objects in the dataset are small, a regime that is notoriously difficult for standard VAE architectures. • Improved representational generalization to out-of-distribution test datasets involving both interpolation and extrapolation in latent space.





% ●	We propose an unconditional Semantic Bottleneck GAN architecture to learn the distribution of complex scenes. To tackle the problems of learning both the global layout and the local structure, we divide this synthesis problem into two parts: an unconditional segmentation map synthesis network and a conditional segmentation-to-image synthesis model. Our first network is designed to coarsely learn the scene distribution by synthesizing semantic layouts. It generates per-pixel semantic categories following the progressive GAN model architecture (ProGAN) [21]. The second network populates the synthesized semantic layouts with texture by predicting RGB pixel values using SpatiallyAdaptive Normalization (SPADE) [32], following the architecture of the state-of-the-art semantic synthesis network in [32]. We assume the ground truth segmentation masks are available for all or part of the target scene dataset. In the following sections, we will first discuss our semantic bottleneck synthesis pipeline and summarize the SPADE network for image synthesis. We will then couple these two networks in an end-to-end final design which we refer to as

% Overall, our work shows how integrating stronger more transparent structure into the generation process is beneficial across multiple key aspects.

%  that reaches enhanced disentanglement
% high 
% Overall, by integrating stronger more transparent structure into the generation process, we
% supporting one-to-many mapping between the layout and the produced images to maintain .

% which manage to avoid feature matching in order to maintain to sample diversity

% In our work, we mitigate this issue by introducing/proposing novel \textit{Semantic-Matching} and \textit{Segment-Fidelity} losses which maintain the one-to-many relation that holds between layouts and images. 
% Beyond the proposed model and explored 
% In developing the model sketching, we 
% to produce discrete laytout
% Technical contributions 

% New architecture: 
% Generating image in two stages: sketching + painting. Disentangles style and structure.
% , which encourages Object disentanglement/controllability. leveraging transformers.
% Unsupervised , .
% 2.5d depth awareness
% encourages amodal completion
% Compositional and iterative generation of the image in a way that accounts for objects / regions

% Contributions

% contribution: 
% disc loss: more accurately enforce complicated geometric constraints on the global image structure.
% structural loss

% - New architecture: Generating image in two stages: sketching + painting. Disentangles style and structure.
% Compositional and iterative generation of the image in a way that accounts for objects / regions, which encourages Object disentanglement/controllability. leveraging transformers.
% - Unsupervised 2.5d depth awareness, encourages amodal completion.

% Better interpretability compared to standard GANs. (ability to debug issues).

% We study the model quantitative and qualitative behavior
% through a series of experiments, where it achieves state-ofthe-art performance over a wide selection of datasets, of
% both simulated as well as real-world kinds, obtaining particularly impressive gains in generating highly-compositional
% multi-object scenes. The analysis we conduct indicates that the GANsformer requires less training steps and fewer samples than competing approaches to successfully synthesize images of high quality and diversity. Further evaluation provides robust evidence for the network’s enhanced transparency and compositionality, while ablation studies empirically validate the value and effectiveness of our approach. We then present visualizations of the model’s produced attention maps to shed more light upon its internal representations and visual generation process. All in all, as we will see through the rest of the paper, by bringing the renowned GANs and Transformer architectures together under one roof, we can integrate their complementary strengths, to create a strong, compositional and efficient network for visual generative modeling.

\begin{comment}

We demonstrate the value and performance of the Neural State Machine on two recent Visual Question
Answering (VQA) datasets: GQA [41] which focuses on real-world visual reasoning and multi-step
question answering, as well as VQA-CP [3], a recent split of the popular VQA dataset [2, 27] that
has been designed particularly to evaluate generalization. We achieve state-of-the-art results on
both tasks under single-model settings, substantiating the robustness and efficiency of our approach
in answering challenging compositional questions. We then construct new splits leveraging the
associated structured representations provided by GQA and conduct further experiments that provide
significant evidence for the model’s strong generalization skills across multiple dimensions, such
as novel compositions of concepts and unseen linguistic structures, validating its versatility under
changing conditions.

We demonstrate the model’s quantitative and qualitative performance on the CLEVR task and its
associated datasets. The model achieves state-of-the-art accuracy across a variety of reasoning tasks
and settings, both for the primary dataset as well as the more difficult human-authored questions.
Notably, it performs particularly well on questions that involve counting and aggregation skills,
which tend to be remarkably challenging for other VQA models (Santoro et al., 2017; Hu et al.,
2017; Johnson et al., 2017b). Moreover, we show that the MAC network learns rapidly and generalizes effectively from an order of magnitude less data than other approaches. Finally, extensive
ablation studies and error analysis demonstrate MAC’s robustness, versatility and generalization
capacity. These results highlight the significance and value of imposing strong structural priors to
guide the network towards compositional reasoning. The model contains structures that encourage
it to explicitly perform a chain of operations that build upon each other, allowing MAC to develop
reasoning skills from the ground up, realizing the vision of an algebraic, compositional model of
inference as proposed by Bottou (2014). Although each cell’s functionality has only a limited range
of possible continuous behaviors, geared to perform a simple reasoning operation, when chained
together in a MAC network, the whole system becomes expressive and powerful. TensorFlow implementation of the model is available at https://github.com/stanfordnlp/mac-network

\end{comment}

 
% decoupling two major tasks;
% General: To overcome these limitations, we propose a new model, the Semantic Bottleneck GAN, which couples high-fidelity generation capabilities of labelconditional models with the flexibility of unconditional image generation. This in turn enables our model to synthesize an unlimited number of novel complex scenes, while still maintaining high-fidelity output characteristic of imageconditional models.

% In analogy to how human painters draw, we decompose the problem of text to photo-realistic image synthesis into two more tractable sub-problems with Stacked Generative Adversarial Networks (StackGAN).

% compositional:segmentation, depth, iterative, combine them together to structured image generation approach 

% objs: 
% They maintain explicit object representations,

% dependens:

% advtanges:

% Why S2 -GAN? We believe there are fourfold advantages of factoring the style and structure in the image generation process. Firstly, factoring style and structure simplifies the overall generative process and leads to more realistic high-resolution images. It also leads to a highly stable and robust learning procedure. Secondly, due to the factoring process, S2 -GAN is more interpretable as compared to its counterparts. 

% extra: lines of work, seeking to be at the same time geometrically rich enough to handle complex object shapes and textures, explicit enough about objects to support the top-down inferential reasoning capacities of generative models, flexible enough to learn from real-world or realistic (not toy) visual data,



\begin{comment}
Motivated to address these shortcomings and unlock the
full potential of this promising network for the field of computer vision, we introduce the Generative Adversarial Transformer, or GANsformer for short, a simple yet effective
generalization of the vanilla transformer, explored here for
the task of visual synthesis. The model features a biparatite
construction for computing soft attention, that iteratively
aggregates and disseminates information between the generated image features and a compact set of latent variables to
enable bidirectional interaction between these dual representations. This proposed design achieves a favorable balance,
being capable of flexibly modeling global phenomena and
long-range interactions on the one hand, while featuring an
efficient setup that still scales linearly with the input size
on the other. As such, the GANsformer can sidestep the
computational costs and applicability constraints incurred
by prior work, due to their dense and potentially excessive
pairwise connectivity of the standard transformer [5, 72],
and successfully advance generative modeling of images
and scenes.


Motivated to alleviate these deficiencies and bring the neural and symbolic approaches more closely
together, we propose the Neural State Machine, a differentiable graph-based model that simulates
the operation of an automaton, and explore it in the domain of visual reasoning and compositional
question answering. Essentially, we proceed through two stages: modeling and inference. Starting
from an image, we first generate a probabilistic scene graph [43, 49] that captures its underlying
semantic knowledge in a compact form. Nodes correspond to objects and consist of structured
representations of their properties, and edges depict both their spatial and semantic relations. Once
we have the graph, we then treat it as a state machine and simulate an iterative computation over
it, aiming to answer questions or draw inferences. We translate a given natural language question
into a series of soft instructions, and feed them one-at-a-time into the machine to perform sequential
reasoning, using attention to traverse its states and compute the answer.

Seeking a balance between the versatility and robustness of end-to-end neural approaches on the
one hand and the need to support more explicit and structured reasoning on the other, we propose
the MAC network, a novel fully differentiable architecture for reasoning tasks. Our model performs
structured and explicit reasoning by sequencing a new recurrent Memory, Attention and Composition (MAC) cell. The MAC cell was deliberately designed to capture the inner workings of an
elementary, yet general-purpose reasoning step, drawing inspiration from the design principles of
computer architectures. The cell explicitly separates out memory from control, both represented
recurrently, and consists of three operational units that work in tandem to perform a reasoning step:
the control unit updates the control state to attend at each iteration to some aspect of a given question; the read unit extracts information out of a knowledge base, guided by the control and memory
states; and the write unit integrates the retrieved information into the memory state, iteratively computing the answer. This universal design of the MAC cell serves as a structural prior that encourages
the network to solve problems by decomposing them into a sequence of attention-based reasoning
operations that are directly inferred from the data, without resorting to any strong supervision. With
self-attention connections between the cells, the MAC network is capable of representing arbitrarily complex acyclic reasoning graphs in a soft manner, while still featuring a physically sequential
structure and end-to-end differentiabillity, amenable to training simply by backpropagation.


% Motivated to ameliorate/mitigate these shortcomings

 It operates in two stages: a fast and lightweight \textit{sketching} phase, where we plan a high-level/global layout of a new scene, followed by an attention-based \textit{painting} phase, where the layout is honed and refined, evolving into a rich and detailed final image. This approach allows us to shift/move away from [the] [standard/typical] traditional/conventional black-box/convolutional [GAN] architectures that feature/use/interact with a flat and monolithic latent space, towards a transparent design that encourages efficiency/efficacy, interpretability, and controllability over the [image/visual] generation process. We demonstrate the model's qualities and strengths through a careful/extensive/comprehensive evaluation over a range of datasets, from simulated multi-object CLEVR scenes on the one end to the challenging and diverse real-world COCO images on the other, showing it successfully achieves state-of-the-art performance in terms of image quality, consistency and fidelity/realism. Further quantitative and qualitative experiments/studies illustrate the additional merits/advantages [and beneficial properties] of the approach/model in terms of adaptability/adaptivity/flexibility, versatility/customization and disentanglement, and provide a deeper insight into its synthesis process, as it proceeds/[successively] progresses [step-by-step] from a rough initial sketch, to a detailed layout that accounts for objects' depths and dependencies, and up to the final high-resolution depiction/portrayals/images of intricate and vibrant real-world scenes.
 
 \end{comment}
 
 
% uto-predicted segmentations (either produced in an unsupervised manner \citep{unsup} for the case of CLEVR \cite{clevr} or using a pre-trained segmentor \cite{detectron2} for real-world images).
% To train the stage, we 

% The number of generated segments per step is variable 
% ***conditioned upon its predecessor 
% panoptic segmentations
% Such that the 
% The generation 
% In the 
% *variable number of objects
% differentaibility

% We [wish to] emphasize the that number of segments (or objects) in the layout is \textit{variable}, and as we see below, the model is indeed capable of producing layouts of a variable size. 
% One important point in which we differ from the original GANsformer regards to the number of latent variables used by the model. While the original GANsformer 
% train this stage over 
% 5) loss (hierarchical noise scheme)
% departs, but rather
% discrimnator description 
% * Sketch generation: new training scheme for discrete output by adding hierarchical noise.

% where we plan a \textbf{scene layout} -- a collection of segments corresponding to objects, regions or entities in the scene. Each segment corresponds to a spatial region, and posses also a soft semantic label (probably distribution over 


% layout: Semantic layout defines a structure of scene based on object instances and provides fine-grained information of the scene, such as the number of objects, object category, location, size, shape, etc.

% conditional disen:
% While the definition of disentanglement is open to debate, many believe a factorial representation, one with statistically independent variables, is a good starting point [1, 2, 3]. Such representations distill information into a compact form which is oftentimes semantically meaningful and useful for a variety of tasks [2, 4]. For instance, it is found that such representations are more generalizable and robust against adversarial attacks [5]. It is also argued that encouraging independence between latent variables induces disentanglement [7].

% Conditional/directed disentanglement: instead of standard disentanglement, which tries to push to independent-axes representation, model representation captures dependencies between the different objects:


% control:
% __________________
% experiments:
% depth proxy!
% ****,
% ubiquitous widespread
% Thanks to the advent / emergence
% ***by interpreting it from multiple abstraction levels. 
% The above process reflects how a human draws a scene by interpreting it from multiple abstraction levels.
% ****
% encode
% capable
% recall uv
% ***ground-truth 
% stark contrast
% __________________

